Efficient Multiscale Gaussian Process Regression using Hierarchical Clustering

Standard Gaussian Process (GP) regression, a powerful machine learning tool, is computationally expensive when it is applied to large datasets, and potentially inaccurate when data points are sparsely distributed in a high-dimensional feature space. To address these challenges, a new multiscale, sparsified GP algorithm is formulated, with the goal of application to large scientific computing datasets. In this approach, the data is partitioned into clusters and the cluster centers are used to define a reduced training set, resulting in an improvement over standard GPs in terms of training and evaluation costs. Further, a hierarchical technique is used to adaptively map the local covariance representation to the underlying sparsity of the feature space, leading to improved prediction accuracy when the data distribution is highly non-uniform. A theoretical investigation of the computational complexity of the algorithm is presented. The efficacy of this method is then demonstrated on smooth and discontinuous analytical functions and on data from a direct numerical simulation of turbulent combustion.

==> analytical0.tex <==
\subsection{Analytical examples}
\begin{figure}[ht]
	\centering
\includegraphics[width=0.7\textwidth]{figures/ana/step1.pdf}
\caption{Comparison of the output of the standard kernel GP (using a Gaussian kernel)
and MGP ($S=1$) for a step function. The crosses are training points ($N=128$), while the continuous lines and shaded
areas show the predictive mean and the variance.}  \label{stepfig1}
\end{figure}

\begin{figure}[ht]
	\centering
\includegraphics[width=0.7\textwidth]{figures/ana/step1b.pdf}
\caption{Comparison of the performance of the standard GP and MGP for the step function in Figure \ref{stepfig1}. The plot on the left shows the size of the extended feature space for different input noise $\sigma$. The
wall clock time is obtained using MATLAB on a typical desktop PC.}  \label{stepfig1b}
\end{figure}

\begin{figure}[ht]
	\centering
\includegraphics[width=0.7\textwidth]{figures/ana/step2.pdf}
\caption{Comparison of the standard GP and MGP for a step function. In contrast to Figure \ref{stepfig1}, the training point distribution is non-uniform with an exponential density increase near the jump. The number of training points $N=101$. Gaussian noise with $\sigma =0.03$
was added. The crosses
represent training points, while the continuous lines and shaded
areas show the predictive mean and the variance. The dots on the continuous
line have abscissas of the training points. }  \label{stepfig2}
\end{figure}

\begin{figure}[ht]
	\centering
\includegraphics[width=0.7\textwidth]{figures/ana/sine1.pdf}
\caption{Comparison of performance of the standard GP and MGP ($S=1$) for a sine function, $y = \sin(2\pi q(4q + 1)^{1.5})$ with Gaussian noise of standard deviation $\sigma = 0.01$. Crosses represent training points ($N=128$); continuous lines and shaded regions show the predictive mean and the variance.}  \label{sinefig1}
\end{figure}

\begin{figure}[ht]
	\centering
\includegraphics[width=0.7\textwidth]{figures/ana/sine2.pdf}
\caption{Comparison of the performance of the standard GP and MGP for the sine function in Figure \ref{sinefig1}. The
wall-clock time is obtained using MATLAB on a typical desktop PC.}  \label{sinefig2}
\end{figure}

The first numerical example we present is a 1-D step function ($d=1$). We
compare the standard kernel GP with a Gaussian kernel and the present MGP
algorithm restricted to a single scale ($S=1$). The training set of size $N$ was randomly selected from 10000 points distributed
in a uniform grid. Points not used for training were used as test points. The initial data was
generated by adding normally distributed noise with standard deviation $%
\sigma$ to the step function. Optimal hyperparameters were found using the Lagarias algorithm for the Nelder-Mead method (as implemented by MATLAB's
\texttt{fminsearch} function) \cite{lagarias}. For the standard GP, $\sigma$
and $h$ were optimized, while for the MGP algorithm, the optimal $\gamma 
$ was determined in addition to $\sigma$ and $h$. In both cases the optimal $\sigma$ was close  to the
actual $\sigma $ used for data generation. The ratio between the optimal $h$ for the kernel and the finite-dimensional
(``weight-space'') approaches was found to be approximately 
$1.4$, which is consistent with the difference of $\sqrt{2}$ predicted by
the theory (see discussion after Eq. (\ref{p15})). 

The plots in Figure \ref{stepfig1} show that there is no substantial
difference in the mean and the variance computed using both methods, while
the sparse algorithm required only $D=38$ functions compared to the $N=128$
required for the standard method. The bottom-left plot shows how $D$
changes with $N$. Ideally, this should be a linear dependence, since the step function is scale-independent. Due to random noise and the fact that the optimization may
converge to local minima of the objective function that are different
from the global optima, the relationship is not exactly linear. Since $D$ is nevertheless several times smaller than $N$ for all $N$, the wall-clock time for the present
algorithm is shorter than that for the standard GP in both testing and training, per optimizer iteration.
The total training time for the present algorithm can be larger than for the standard algorithm due to the overhead related to the larger number of hyperparameters and the resultant increase in the number of optimization iterations required. 
%The total training time for the present algorithm can be larger than for the standard algorithm due to the overhead related to reducing the size of the problem from $N$ to $D$ through the clustering algorithm. 
However, we observed this only for
relatively small values of $N$. For larger $N$, such as $N=4096$, the present
algorithm was approximately 5, 10, and 20 times faster than the standard
algorithm for $\sigma =0.1$, $0.01$, and $0.001$, respectively.

Figure \ref{stepfig2} illustrates a case where the training points are distributed non-uniformly. Such situations
frequently appear in practical problems, where  regions of high functional gradients are sampled with higher density to provide a good representation of the function. For example, non-uniform meshes for capturing shockwaves and boundary layers in fluid flow fall into this category. In the case illustrated here, the training points were
distributed with exponential density near the jump ($q=0.5\pm h_{t}\ln z$, $%
\exp \left( -0.5/h_{t}\right) \leqslant z\leqslant 1$, where $z$ are
distributed uniformly at the nodes of a regular grid. $h_{t}=0.1$ was used). For MGP, the number of scales was $S=6$
and the other hyperparameters were optimized using the same routine as before. Due to multiple extrema in the objective function, it is rather difficult to optimize the number of \ scales, $S$. In practice, one should start from several initial guesses or fix some parameters such as $S$. We used several values of $%
S$ and observed almost no differences for $5\leq S \leq 10$,
while results for $S=1$ and $S=2$ were substantially different from the cases where $S>2$.

It is seen that the MGP provides a much better fit of the step
function in this case than the standard method. This is achieved due to its
broad spectrum of scales. In the present example we obtained the following
optimal parameters for scales distributed as a geometric progression, $%
h_{s}=h_{1}\beta ^{s-1}$: $h_{\max }=h_{1}=0.1233$, $h_{\min }=h_{6}=0.0032$%
, and $\beta =0.4806$. Other optimal parameters were $\gamma =0.258$ and $\sigma
=0.127$. For the standard GP, the optimal scale was $h=0.0333$. Figure \ref{stepfig2}
shows that with only a single intermediate scale, it is impossible to
approximate function between training points with a large spacing, whereas MGP provides a much better approximation.
Moreover, since $h_{\min }<h$, we also have a better approximation of the jump, i.e. of
small-scale behavior. This is clearly visible in the figure; the jump for
the standard GP is stretched over about 10 intervals between sampling
points, while the jump for MGP only extends over 3 intervals.
Note that in the present example, we obtained $D=N=101$, so the
wall-clock time for testing is not faster than the standard GP. However, this case
illustrates that multiple scales can provide good results for substantially
non-uniform distributions where one scale description is not sufficient. 

A final analytical example we present prior to testing on data from engineering applications is that of a sine wave with varying frequency, depicted in Figure \ref{sinefig1}. As before, $N$ training points are randomly chosen from a uniform distribution, and $M=10000-N$ test points are used. For MGP, $S=1$ was used. Compared to the previous examples, this is an intermediate case in terms of scale dependence. One noteworthy result from this dataset is that $D$ is almost constant with respect to $N$, as seen in Figure \ref{sinefig2}. This shows that when the function is relatively smooth, the optimization process is not limited to producing a linear relationship between $D$ and $N$. Another result is that the output variance of the multiscale method is visibly higher than that of the standard method. For the previous cases, the variances have been either been close to equal, or the standard method would produce the higher variance. This could be due to the fact that $h$ and $D$ are inherently related for the current method, whereas $h$ is unrestricted for the standard GP. Since $D<N$, the multiscale $h$ for $S=1$ is typically greater than the standard method's $h$. According to Eqs. (\ref{p11}) and (\ref{p15}), this would result in greater variance. 



==> analytical1.tex <==
\subsection{Analytical example}
The first example considers a simple one-dimensional noisy sine function, $y = \sin(8\pi q) + \mc{N}(0,0.1)$, with $q \in [0,1]$. Two cases are tested: the first with training values for $q$ chosen from a uniform distribution, and the second with $q$ chosen randomly from normal distributions centred around $0.1$, $0.5$, and $0.9$. 300 training points are used in each case. Prior to usage in GP, training inputs and outputs are scaled to $[0,1]$. Test inputs are scaled using the range and minimum of $\mb{Q}_{\mr{train}}$, and the results from learning are scaled back using the range and minimum of $\mb{Y}_{\mr{train}}$.

As in Figure \ref{mgp2d1} in the previous section, Figures \ref{sinerand} and \ref{sinerandn} further illustrate the process of selecting cluster centres. These figures represent the uniform and clustered input cases, respectively. In each figure, the plot on the left shows the cluster centres chosen using $h_k=h_1=0.1$, the middle plot with $h_2=0.05$, and the right plot with $h_3=0.025$. Since $h_k$ decreases with $k$, more centres are chosen with increasing $k$ because they are not constrained to be as far apart from each other. The centres are randomly chosen, such that they are not evenly distributed across the domain, but the spacing between them is close to $h_k$ at each $h_k$. With these sample parameters, approximately 50 centres are selected cumulatively across these three scales, and the rest of the training points are disregarded. This means the size of the training dataset has effectively been reduced from 300 to 50. The consequent benefits in training and testing costs are evident.

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerand.pdf}
		\caption{Clustering produced by MGP for uniform distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points, signifying points that were within $h_k$ of the cluster centre at the time of its selection. $h_0=0.1$, $r = 2$. } \label{sinerand}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerandn.pdf}
		\caption{Clustering produced by MGP for clustered distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points within $h_k$ of the centre. $h_0=0.1$, $r = 2$ as before. }  \label{sinerandn}
\end{figure}

Following the cluster selection, the optimal hyper-parameters for each method are found through minimizing the LML, and the results of testing on new sets of randomly selected $q_{\mr{test}}$ using the optimized ML methods are summarised in Table \ref{sineerr}. No validation sets were used, meaning that all the original training points were considered when computing the LML. For the clustered case, MGP used only 20 cluster centres out of 300 original training points to achieve this result, plotted in Figures \ref{sineures} and \ref{sinecres}. Despite the more than ten-fold reduction in the number of cluster centres vesus the number of training points, the speedup is not precisely linear due to computational overhead. Figures \ref{sineuline} and \ref{sinecline} depict the ML output $f(q_{\mr{test}})$ versus the original $y_{\mr{test}}$. In general, the variance of the output appears larger near the extrema of the sine function and smaller near zero, the same behaviour as observed in Figures \ref{sineures} and \ref{sinecres}.

\begin{table}
\caption{Normalised test errors for ML methods, defined as $||\mb{Y}_{\mr{test}} - f(\mb{Q}_{\mr{test}})||/||\mb{Y}_{\mr{test}}||$. 1000 uniformly spaced test points on $[0,1]$ were used.  Time is test time in seconds.}
\label{sineerr}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Uniform input & 0.0257 & $7.7\times10^{-3}$ & 0.0407 & $2.4\times10^{-3}$ \\ \hline
    Clustered input & 0.0516 & $9.6\times10^{-3}$ & 0.0716 & $1.7\times10^{-3}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sineuniform.pdf}
		\caption{Uniform distribution testing results for all methods. Black line is the original function, black dots are training points with noise added. Blue line is the ML output. For GP and MGP, shaded red regions indicate confidence intervals of $\pm1\sigma$. }  \label{sineures}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinecluster.pdf}
		\caption{Clustered distribution testing results for all methods. Black line is the original function, black dots are training points. Blue line is the ML output. For GP and MGP, red regions are confidence intervals of $\pm1\sigma$. There are noticeable divergences from the true function, especially near maxima and minima, compared to the uniformly distributed training point case.}  \label{sinecres}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandline.pdf}
		\caption{Test output $y_{\mr{test}}$ versus ML output $f(q_{\mr{test}})$ for uniformly distributed test points. The red line is $f(q_{\mr{test}}) = y_{\mr{test}}$. Shaded red region is $\pm 0.1$ from the red line, i.e. one standard deviation for the noise in the training data.}  \label{sineuline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandnline.pdf}
		\caption{$y_{\mr{test}}$ versus $f(q_{\mr{test}})$ for clustered test points. Red line is $f(q_{\mr{test}}) = y_{\mr{test}}$, shaded red region is $\pm 0.1$ from the red line. Ordinary GP is clearly deviating from the line, likely in locations lacking training points.}  \label{sinecline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08.pdf}
		\caption{Tradeoffs in speed and accuracy for performing MGP on uniformly distributed data. Blue points are for randomly-selected hyperparameters, and orange `x's are for using the optimal hyperparameters from maximizing the LML. The two plotted have $K=5$ and $K=6$, with the former having less error. The black `x' is a sample GP for comparison. The error for MGP rises very sharply as test time decreases beyond a certain point.}  \label{sineupareto}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08randn.pdf}
		\caption{Tradeoffs in speed and accuracy for MGP on clustered data. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=5$ and $K=6$, the former having lower error. Black is a sample GP result for comparison.}  \label{sinecpareto}
\end{figure}

As a final note, Figures \ref{sineupareto} and \ref{sinecpareto} show that parameters selected through maximizing the LML are also near optimal according to the test error, validating the use of LML for hyperparameter optimization. Comparing this to the numerical results in Table \ref{sineerr}, the tradeoff between speed and accuracy is shown to be worthwhile for the majority of cases, since the percentage decrease in test time is greater than the increase in error. As number of scales $K$ increases, the test error increases sharply for the clustered training data, but does not increase much for the evenly distributed training data. In addition, for $K<5$, the test error also increases rapidly to the point where the optimal results for $K\leq4$ are not visible in the figures. This suggests the tendency to overfit using MGP, and the risk of selecting 
too few training points. 

%\begin{itemize}
%\item Is it helpful to compute average error and speedup from different random sets of training points, or is the scatterplot sufficient?
%\end{itemize}

==> bibliography.tex <==
\begin{thebibliography}{99}% maximum number of references (for label width)
 %\bibitem{rebek:82bk}
 %Rebek, A., {\it Fickle Rocks}, Fink 
 %Publishing, Chesapeake, 1982.
 \bibitem{spalart}
 Spalart, P. R. and Allmaras, S. R., ``A One-Equation Turbulence Model for Aerodynamic Flows,'' {\it 30th Aerospace Sciences Meeting \& Exhibit,}, Reno, NV, Jan. 1992.
 
  \bibitem{kom}
  Wilcox, D., {\it Turbulence modeling for CFD}, Vol. 2, DCW industries, 2006.
 
  %SARC derivation
 %\bibitem{sarcemp}
 %Spalart, P. R. and Shur, M., ``On the sensitization of turbulence models to rotation and curvature,'' {\it Aerospace Science and Technology}, Vol. 1, No. 5, 1997, pp. 297-302.
 
  % learning kom constants
 \bibitem{komlearn}
 Yarlanki, S., Rajendran, B., and Hamann, H., ``Estimation of turbulence closure coefficients for data centers using machine learning algorithms,'' {\it 13th IEEE Intersociety Conference on Thermal and Thermomechanical Phenomena in Electronic Systems}, May 2012.
 
  % learning velocity field
 \bibitem{vellearn}
 Milano, M. and Koumoutsakos, P., ``Neural network modeling for near wall turbulent flow,'' {\it Journal of Computational Physics}, Vol. 182, No. 1, 2002, pp. 1-26.
 
 % similar to us but for LES SGS model
 \bibitem{lessgs}
 Sarghini, F., de Felice, G., and Santini, S., ``Neural networks based subgrid scale modeling in large eddy simulations,'' {\it Computers \& Fluids}, Vol. 32, No. 1, 2003, pp. 97-108.
 
  %SARC
 %\bibitem{sarc}
 %Shur, M. L., Strelets, M. K., Travin, A. K., and Spalart, P. R., ``Turbulence modeling in rotating and curved channels: Assessing the Spalart-Shur correction,'' {\it AIAA Journal}, Vol. 38, No. 5, 2000, pp. 784-792.
 \bibitem{transitionref}
 Ge, X., Arolla, S., and  Durbin, P., ``A bypass transition model based on the intermittency function,'' {\it Flow, Turbulence and Combustion}, Vol.
93, No. 1, 2014, pp. 37–61.
 
 
 \bibitem{inverseref1}
 Aster, R. C., Borchers, B., and Thurber, C. H., {\it Parameter estimation and inverse problems,} Academic Press, 2013.
 
 \bibitem{inverseref2}
 Isaac, T., Petra, N., Stadler, G., and Ghattas, O., ``Scalable and efficient algorithms for the propagation of uncertainty
from data through inference to prediction for large-scale problems, with application to flow of the Antarctic ice sheet,'' {\it arXiv
preprint,} arXiv:1410.1221, 2014.

  %Eric's paper
 \bibitem{eric}
 Parish, E. and Duraisamy, K., ``Quantification of Turbulence Modeling Uncertainties Using Full Field Inversion,'' {\it 15th AIAA Aviation Technology, Integration, and Operations Conference,}, Dallas, TX, June 2015.
 
  \bibitem{transprev}
 Duraisamy, K., Zhang, Z., and Singh, A., ``New Approaches in Turbulence and Transition Modeling Using
Data-driven Techniques,'' {\it AIAA Modeling and Simulation Technologies Conference,}, Kissimmee, FL, January 2015.
 
 \bibitem{mlbook}
 Bishop, C. M., {\it Pattern Recognition and Machine Learning,} Springer, 2006.
 
 \bibitem{hillclimb}
 Kohavi, R. and John, G. H., ``Wrappers for Feature Subset Selection,'' {\it Artificial Intelligence,} Vol. 97, No. 1, 1997, pp. 273-324.
 
 \bibitem{fannlib}
 Nissen, S., ``Fast Artificial Neural Network Library - FANN.''
 
 \bibitem{rbfgp1}
 Park, J. and Sandberg, I. W., ``Universal Approximation Using Radial-Basis-Function Networks,'' {\it Neural Computation,} Vol. 3, No. 2, 1991, pp.246-257.
 
 \bibitem{rbfgp2}
 Rasmussen, C. E. and Williams, C. K. I., {\it Gaussian Processes for Machine Learning,} MIT Press, 2006.
 
 \bibitem{mgpcomm}
 Gumerov, N. A. and Duraisamy, K., private communication, University of Maryland, College Park, MD, Sept. 2014.
 
%alternate MGP paper
\bibitem{mgppaper}
Walder, C., Kim, K. I., and Schölkopf, B., ``Sparse multiscale Gaussian process regression,'' {\it Proceedings of the 25th international conference on Machine learning}, July 2008.

%[snelson Ghahramani sparse GP pseudoinput] http://papers.nips.cc/paper/2857-sparse-gaussian-processes-using-pseudo-inputs.pdf

%[same authors, local and global sparse GP]http://mlg.eng.cam.ac.uk/zoubin/papers/aistats07localGP.pdf

%[GP research review paper] http://jmlr.org/papers/volume6/quinonero-candela05a/quinonero-candela05a.pdf

%[extension to above by different group] http://www.cyberneum.de/fileadmin/user_upload/files/publications/lskm_chap_%5B0%5D.pdf

%[smola bartlett greedy sparse GP]http://citeseerx.ist.psu.edu/viewdoc/summary?doi=10.1.1.19.8811

%[random features for kernel]http://www.eecs.berkeley.edu/~brecht/papers/07.rah.rec.nips.pdf

%[urtasun darrell local GP]http://mplab.ucsd.edu/wp-content/uploads/CVPR2008/Conference/data/papers/020.pdf

%[titsias 2009]http://jmlr.org/proceedings/papers/v5/titsias09a/titsias09a.pdf

%[seeger 2003]http://ipg.epfl.ch/~seeger/lapmalmainweb/papers/aistats03-final.pdf

%[keane parallel GP with clusters]http://epubs.siam.org/doi/pdf/10.1137/1.9781611972726.6

%[weiss, GPU parallel GP demo]http://arxiv.org/pdf/1310.5182v2.pdf



\end{thebibliography}

==> gp_Orig.tex <==
\section{Background}
In machine learning, an algorithm is trained using existing data so that it can be tested by making predictions on new data.  For applications of regression, the dataset consists of sets of points $(\mb{q},y)$, where the input vector $\mb{q} \in\mathbb{R}^{d}$, and the output vector $y\in\mathbb{R}^{c}$. Given a set of $N$ outputs $\mathbf{Y}\in \mathbb{R}^{N\times c}$ and its corresponding set of $N$ inputs $\mathbf{Q}\in \mathbb{R}^{N\times d}$, it is customary\cite{mlbook} to divide them into training and validation sets, $(\mathbf{Q}_{\mr{train}},\mathbf{Y}_{\mr{train}})$ and $(\mathbf{Q}_{\mr{val}},\mathbf{Y}_{\mr{val}})$. These sets consist of $N_{\mr{train}}$ and $N_{\mr{val}}$ points, respectively. A ML algorithm is first applied to the training set to obtain the function $f$, where $f(\mathbf{q})\approx y$. Then, the error on the validation set can be used to adjust any hyperparameters the ML algorithm may possess. Once this is done, the algorithm can be tested by evaluating $f(\mathbf{q}_{\mr{test}})$ and comparing the result with $y_{\mr{test}}$.

In the description that follows, the output $y$ is scalar and assumed to be noisy, generated by adding ideally Gaussian noise with variance $\lambda$ to an original function $y_0$,
\begin{equation}
y(\mb{q}) = y_0(\mb{q}) + \mc{N}(0,\lambda)
\end{equation}
Obtaining the variance of the ML output $f$, $\sigma^2_f$ is very straightforward when $\lambda$ is known originally. Even without that information, $\lambda$ and $\sigma^2_f$ can be estimated, as will be shown later.

A GP assumes that the output at the training points, $\mb{Y}_{\mr{train}}$, is drawn from the distribution
\begin{equation}
\mb{Y}_{\mr{train}} \sim \mc{N}(\mb{0},\mb{\Phi} + \lambda\mb{I})
\end{equation}
$\mb{\Phi}$ is a matrix of covariances between training points. The mean of the distribution is unknown, so it is set to zero. The posterior after the incorporation of data is not limited by any particular prior; setting the mean to zero is for ease of computation only. The noise of the output is added to the covariance between training points because they are assumed to be independent. The current work employs a radial basis function (RBF)\cite{rbfgp1}$^,$\cite{rbfgp2} kernel for computing GP covariance:
\begin{equation}
\mb{\Phi}(m,n) = \phi(\mathbf{q}_m,\mathbf{q}_n) = e^{-\frac{||\mathbf{q}_m - \mathbf{q}_n||^2}{h^2}}
\label{GPeqn}
\end{equation} 
where $\mb{q}_m$, $\mb{q}_n$ are points from $\mb{Q}_{\mr{train}}$. Since the covariance matrix must be populated by computing the value of the the kernel function between all possible pairs of training points, it is now evident that computing the output of a GP depends on the size of the training set. Also, note that points that are closer in input space are assumed to be more correlated, and points that are further, less.

Given a test point $\mb{q}_{\mr{test}}$, the corresponding $f(\mb{q}_{\mr{test}})$ can be defined via a conditional probability distribution, $p(f|\mb{Y}_{\mr{train}})$. The mean of this distribution is the predicted value of $f$ given the training points, and the variance is $\sigma^2_f$. Using standard probability formulae
\[\mu_{a|b} = \mu_a + \Sigma_{ab}\Sigma_{bb}^{-1}(y_b - \mu_b)\]
\[\Sigma_{a|b} = \Sigma_{aa} - \Sigma_{ab}\Sigma_{bb}^{-1}\Sigma_{ba}\]

it is found that 
\begin{equation}
p(f|\mb{Y}_{\mr{train}}) \sim \mc{N}(\underline{\phi}^T(\mb{\Phi} + \lambda\mb{I})^{-1}\mb{Y}_{\mr{train}}, 1+\lambda-\underline{\phi}^T(\mb{\Phi} + \lambda\mb{I})^{-1}\underline{\phi})
\end{equation}
and hence, both the expected value and variance of $f$ are obtained:
\begin{eqnarray}
f = \underline{\phi}^T(\mb{\Phi} + \lambda\mb{I})^{-1}\mb{Y}_{\mr{train}} \\
\sigma^2_f = 1+\lambda-\underline{\phi}^T(\mb{\Phi} + \lambda\mb{I})^{-1}\underline{\phi}
\label{yvareqn}
\end{eqnarray}
$\underline{\phi}$ is a vector whose elements are $\phi(\mb{q}_{\mr{train},i},\mb{q}_{\mr{test}})$, with $\mb{q}_{\mr{train},i}$ being the $i$th data point in $\mb{Q}_{\mr{train}}$. Given the form of the kernel function, the value of $f$ will be closer to the values of $y_{\mr{train}}$ for which $\mb{q}_{\mr{train}}$ is close to $\mb{q}_{\mr{test}}$.

In cases where $\lambda$ is supplied, $\sigma^2_f$ can be found directly. If there is a different $\lambda$ assigned to each $y_{\mr{train}}$, the scalar $\lambda$ may be replaced by the vector $\mb{\Lambda}$ consisting of all the individual variances at the training points, and the rest of the equations would still hold. In cases where $\lambda$ is unknown, it can be estimated by maximising the log marginal likelihood (LML):
\begin{equation}
\log p(\mb{Y}_{\mr{train}}|\mathbf{Q}_{\mr{train}},h,\lambda) = - \frac{1}{2} \log |\mathbf{\Phi} + \lambda\mb{I}| - \frac{1}{2} \mathbf{Y}^T_{\mr{train}}(\mathbf{\Phi}+\lambda\mb{I})^{-1}\mathbf{Y}_{\mr{train}} -\frac{N_{\mr{train}}}{2}\log(2\pi)
\end{equation}
The LML measures the probability that an estimate of the hyperparameters $h$ and $\lambda$ would yield a distribution that produces $\mb{Y}_{\mr{train}}$ when sampled at $\mb{Q}_{\mr{train}}$, so maximising it would mean finding the most suitable values for $h$ and $\lambda$. 

The computational complexity of GPs is tied to solving the equation
\begin{equation}
\left( \mb{\Phi}+\lambda\mb{I}\right) \mathbf{\gamma =\beta } \label{generalmatrix}
\end{equation}
For a given training set ($\mb{\beta} = \mb{Y}_{\mr{train}}$), the equation must be solved to obtain the predictive mean at the test point.
In addition, the equation with $\mathbf{\beta} =\underline{\phi}$ must be solved again to obtain the predictive variance. Computation of the determinant $|\mathbf{\Phi} + \lambda\mb{I}|$ for the LML can also be costly.

Several algorithms can be applied here. For example,
an algorithm based on the Cholesky decomposition of matrix $\mathbf{\Phi} + \lambda\mb{I}$ is one well-known approach\cite{chol}. The computational complexity of Cholesky decomposition
is $O\left( N_{\mr{train}}^{3}\right) $. Hence, computation of the LML using this
algorithm costs $O(N_{\mr{train}}^{3})$, which is also the cost of the computation of $%
\mathbf{\gamma }$ for the training set. Therefore, the total complexity of
computation of the predictive mean at $N_{\mr{test}}$ test points will be $O\left(
N_{\mr{train}}^{3}+N_{\mr{train}}N_{\mr{test}}\right) $, assuming that the cost of the $N_{\mr{train}}\times N_{\mr{test}}$ matrix-vector
product is $N_{\mr{train}}N_{\mr{test}}$. The total complexity of computation of the predictive
variance at $N_{\mr{test}}$ test points will be $O\left( N_{\mr{train}}^{3}+N_{\mr{train}}^{2}N_{\mr{test}}\right) $ under the
same assumptions.

In order so that the input space is adequately covered by training points, $N_{\mr{train}}$ should be as large as possible. In this light, the above complexity cannot be acceptable for the majority of practical applications. The goal, then, is to
develop algorithms of lower computational complexity.  Ideally, these algorithms should also have good
parallelisation properties so that they can be efficiently executed on advanced
computing architectures. 

In the construction of the kernel matrix, $||\mathbf{q}_m - \mathbf{q}_n||^2$ is the Eucidean distance in $\mathbb{R}^{d}$. It should
be noticed that if $h\ll \min ||\mathbf{q}_m - \mathbf{q}_n||^2 $, then the system matrix $\mb{\Phi}+\lambda\mb{I}$ becomes diagonal, and the solution of the
problem is fast and efficient. Moreover, for cases where $h\lesssim \min ||\mathbf{q}_m - \mathbf{q}_n||^2 $, the problem can be also solved
efficiently using iterative methods (such as the conjugate gradient method). Indeed, in
this case the condition numbers of the system are moderate, while the
matrix-vector product, $\mathbf{\Phi\gamma }$, can be computed efficiently
using algorithms for the Fast Gauss Transform (FGT) \cite{greengard1991},\cite{yang2003}. In this case, the complexity of solution of Eq. \ref{generalmatrix} reduces from $O\left( N_{\mr{train}}^{3}\right) $ to $O\left( N_{\mr{iter}}N_{\mr{train}}\right) $,
where $N_{\mr{iter}}\ll N_{\mr{train}}$ is the number of iterations. It can also be seen 
that computation of the predictive mean and variance at $N_{\mr{test}}$ points reduces
to $O\left( N_{\mr{iter}}N_{\mr{train}}+N_{\mr{test}}\right) $ and $O\left( N_{\mr{iter}}N_{\mr{train}}N_{\mr{test}}\right) $,
respectively, if using the FGT for the respective matrix-vector products.
Similar computational complexities hold for arbitrary $h$ and not very small values of the noise $\lambda$. In this case, $\lambda$ serves as Tikhonov's regularization parameter \cite{tikhonov1977} (refer to the Appendix for details), and
ensures the well-posedness of the problem. Hence,
in all cases indicated above, a reduction of complexity for solution of the
order of $N_{\mr{train}}$ times or even more can be expected, which for large enough $N_{\mr{train}}$
brings many orders of magnitude of acceleration. It is also important to note that
the FGT is a highly parallelisable algorithm \cite{sampath2010}, which shows that efficient
hardware accelerations are also possible in this case.

In contrast, the major challenge is related to treatment of
cases with large enough $h$, $h\gg \min ||\mathbf{q}_m - \mathbf{q}_n||^2 $ and small enough $\lambda$. In this case, the condition
number of the system becomes very large and the problem in Eq. \ref{generalmatrix} becomes
singular or ill-posed. Iterative methods as proposed
above tend to converge very slowly, if at all. Unfortunately, due to the high dimensionality of the input space in many applications, these circumstances hold true for a large number of points $\mb{q}$ since they are distributed sparsely within this space. Depending on the source of the data, $\lambda$ could also be very small. Furthermore, due to the ill-posedness of the problem, small variations
in the input data or noise in the training ($\mathbf{\beta }$) set result in
large variations in solution $\left( \mathbf{\gamma }\right) $ of Eq. \ref{generalmatrix}. Even exact methods for solving linear systems normally demonstrate substantially large numerical errors due to roundoffs in these cases.
Such errors become worse if approximate matrix-vector products, such as
provided by the FGT, are used, even in preconditioned systems. This has two
consequences. First, not exact, but approximate matrix inversion (or approximate solutions of Eq. \ref{generalmatrix}) makes sense in this context. Such solutions should
have a large variation in $\mathbf{\gamma}$ for given $\mathbf{\beta }$. 
Second, approximate function representations can be constructed and used for low-rank system matrix decompositions. 

Much effort has been devoted to the construction of such approximations. Among these is the family of methods of sparse Gaussian process regression. These methods seek to strategically reduce the size of the training set or find appropriate sparse representations of the correlation matrix $\mb{\Phi}$ through the use of induced variables. Descriptions for several methods of this family are provided by Qui{\~n}onero-Candela et. al. \cite{quinonero2005}, who define induced variables $\mb{U}\in \mathbb{R}^{M\times d}$, $\mb{V}\in \mathbb{R}^{M}$ such that

\begin{equation}
p(f|\mb{U}) \sim \mc{N}(\underline{\phi}_u^T\mb{\Phi}_u^{-1}\mb{V}, 1+\lambda-\underline{\phi}_u^T\mb{\Phi}_u^{-1}
\underline{\phi}_u)
\end{equation}

where $\underline{\phi}_u$ is a vector whose elements are $\phi(\mb{u}_i,\mb{q}_{\mr{test}})$, and $\mb{\Phi}_u(m,n) = \phi(\mathbf{u}_m,\mathbf{u}_n)$. From this, it is evident that if $M<N$, the matrix inversion will be less costly to perform. 

It can be difficult to decide upon an optimal algorithm to determine the induced variables that represent the training set best, and these algorithms introduce additional computational cost. The most basic method to select them is to randomly select a fraction of points and define them as the new training set, i.e. choosing $(\mb{U},\mb{V})$ from $(\mb{Q}_{\mr{train}},\mb{Y}_{\mr{train}})$. Seeger \cite{seeger2003}, Smola \cite{smola2001}, and others have developed  selection methods that provide better test results compared to random selection. These methods often depend on optimising modified likelihoods based on $(\mb{U},\mb{V})$ or on approximating the true LML \cite{titsias2009}. Methods that introduce new induced variables instead of choosing from training points can involve solving optimisation problems, again requiring the user to consider the additional computational resources required. 

In addition to choosing the inducing variables, one may also change the form of the covariance matrix. For example, if 
\[\mb{\Psi}_{\mb{a},\mb{b}} \equiv \underline{\phi}_{\mb{a},\mb{u}}\mb{\Phi}_u^{-1}\underline{\phi}_{\mb{b},\mb{u}}^T\]
with $\underline{\phi}_{\mb{a},\mb{u}}(m,n) = \phi(\mathbf{a}_m,\mathbf{u}_n)$, then one can compute the new estimate as \cite{quinonero2005}

\begin{multline}
p(f|\mb{Q}_{\mr{train}}) \sim \mc{N}\left(\mb{\Psi}_{\mb{Q}_{\mr{train}},\mb{q}_{\mr{test}}}^T\left( \mb{\Psi}_{\mb{Q}_{\mr{train}},\mb{Q}_{\mr{train}}} + \lambda\mb{I} \right)^{-1}\mb{Y}_{\mr{train}}, \right.\\ 
\left. \mb{\Psi}_{\mb{q}_{\mr{test}},\mb{q}_{\mr{test}}}+\lambda-\mb{\Psi}_{\mb{Q}_{\mr{train}},\mb{q}_{\mr{test}}}^T\left(\mb{\Psi}_{\mb{Q}_{\mr{train}},\mb{Q}_{\mr{train}}} + \lambda\mb{I}\right)^{-1}
\mb{\Psi}_{\mb{Q}_{\mr{train}},\mb{q}_{\mr{test}}}\right)
\end{multline}
This is equivalent to changing the definition of the covariance from $\phi$ to $\phi'$, where
\[\phi'(\mb{q}_m,\mb{q}_n) = \phi(\mb{q}_m,\mb{U})\mb{\Phi}_u^{-1}\phi(\mb{q}_n,\mb{U})^T\]
Unlike in the case where only a subset of training data is used, all training points are considered, and the matrices are only of rank $M$. There are many variations on this type of manipulation of the covariance. Alternatively, one can approximate $\mb{\Phi}$ directly by taking random samples of the kernel, which is described in \cite{recht2007}. Altering the correlation matrix can cause various undesirable behaviours when computing the test variance, since some matrices no longer correspond to a Gaussian process mathematically. 

Other methods of speeding up GP regression focus on dividing the training set into smaller sets of more manageable size. Snelson and Ghahramani \cite{snelson2007local} employ a local GP consisting of points in the neighbourhood of the test point in addition to a simplified global estimate to improve test results. Urtasun and Darrell \cite{urtasun2008} use the local GP directly, without the induced variables. However, this means test points must either be assigned to a precomputed neighbourhood of training points, as in the former publication, or points must be found on-line for every test point, as in the latter. Both can be quite expensive depending on training set size, though massive parallelisation may mitigate the cost in some aspects \cite{keane2002} \cite{weiss2014}.

Overall, the changes that need to be made to the GP depend upon the resources at hand and the problem that is being addressed. For on-line applications, the main necessity is test speed. However, it would be unwise to ignore training requirements even though training takes place off-line, since the input space is large and new training data may have to be incorporated relatively quickly; time and memory usage must both be taken into account. Therefore, in the next section, a new alteration to GP that could address these specific areas will be introduced.


\textcolor{red}{
Background section
\begin{itemize}
\item Not sure if the last part sufficiently ties in to MGP
\end{itemize}
}

==> gp_new.tex <==

\section{Preliminaries of GP regression}
In this section, a brief review of standard GP regression is presented. While a
detailed review can be found in the excellent book by Rasmussen~\cite{rbfgp2},
the description and notations below provide the necessary context for the development
of the multiscale algorithm proposed in this paper. 

To cast the present method to the general
theoretical framework, we consider the finite dimensional weight-space view
and the infinite dimensional function-space view as in Rasmussen~\cite{rbfgp2}. 
Given a
training set $\mathcal{D}$ of $N$ observations, $\mathcal{D}=\left\{ \left( 
\mathbf{q}_{n},y_{n}\right) \text{ }|\text{ }n=1,...,N\right\} $, where $%
\mathbf{q}_{n}\in \mathbb{R}^{d}$ is an input vector and $y$ is a scalar
ouput, the goal is to obtain the predictive mean, $%
m_{\ast }$, and variance, $v_{\ast }$, at an arbitrary test point $\mathbf{q}%
_{\ast }\in \mathbb{R}^{d}$. Training inputs are collected in the design
matrix $Q\in \mathbb{R}^{d\times N}$ and the outputs form vector $\mathbf{%
y\in }$ $\mathbb{R}^{N}$. It is assumed further that%
\begin{equation}
y=f\left( \mathbf{q}\right) +\epsilon ,\quad \epsilon \sim \mathcal{N}%
(0,\sigma ^{2}),  \label{p1}
\end{equation}%
where $\epsilon $ is Gaussian noise with zero mean and variance $\sigma ^{2}$.

\subsection{Weight-space view}

The standard linear regression model presents $f\left( \mathbf{q}\right) $
in Eq. (\ref{p1}) as

\begin{equation}
f\left( \mathbf{q}\right) =\mathbf{q}^{T}\mathbf{w,}  \label{p2}
\end{equation}%
where $\mathbf{w\in }$ $\mathbb{R}^{d}$ is the vector of weights. In Bayesian analysis, one
specifies a prior and computes the posterior distribution. Particularly, if
the prior distirbution of the weights is  a multivariate Gaussian with zero
mean and covariance matrix $\Sigma _{p}$, then the posterior distribution is
also a multivariate Gaussian with mean $\overline{\mathbf{w}}$ and covariance
matrix $\Sigma $, 
\begin{equation}
\overline{\mathbf{w}}=\frac{1}{\sigma ^{2}}\Sigma Q\mathbf{y,\quad }\Sigma
^{-1}=\frac{1}{\sigma ^{2}}QQ^{T}+\Sigma _{p}^{-1}.  \label{p3}
\end{equation}

Certainly, for low dimensionality $d$ of the inputs, linear regression
cannot satisfy a variety of dependences encountered in practice. For this
case, mapping of the input into high dimensional feature space $\mathbb{R}%
^{D},$ $D>d$ is used and the linear regression model is applied in this
space. Denoting the mapping function $\mathbf{\phi }\left( \mathbf{q}\right) 
$, $\mathbf{\phi }:\mathbb{R}^{d}\rightarrow \mathbb{R}^{D}$ we have%
\begin{equation}
f\left( \mathbf{q}\right) =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}%
\mathbf{w=}\sum_{j=1}^{D}w_{j}\phi _{j}\left( \mathbf{q}\right) \mathbf{%
,\quad w}=\left( w_{1},...,w_{D}\right) \in \mathbb{R}^{D}.  \label{p4}
\end{equation}%
%The analysis in this case is similar to that for the linear regression.
%Particularly, 
The covariance matrices $\Sigma _{p}$ and $\Sigma $ have sizes 
$D\times D$ instead of $d\times d$ and the design matrix $Q$ should be
replaced by matrix $\Phi \in \mathbb{R}^{D\times N}$ with columns $\mathbf{%
\phi }\left( \mathbf{q}_{n}\right) $ instead of $\mathbf{q}_{n}$, $n=1,...,N.
$ The predictive mean and the covariance matrix can then be computed as%
\begin{equation}
\overline{\mathbf{w}}=\frac{1}{\sigma ^{2}}\Sigma \Phi \mathbf{y,\quad }%
\Sigma ^{-1}=\frac{1}{\sigma ^{2}}\Phi \Phi ^{T}+\Sigma _{p}^{-1}.
\label{p5}
\end{equation}%
The Bayesian formalism also provides Gaussian distributions for the training
outputs, and for the predictions,%
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,\Sigma _{l}),\quad y_{\ast }\sim \mathcal{N}%
(m_{\ast },v_{\ast }),  \label{p6} \\
\Sigma _{l}^{-1} &=&\frac{1}{\sigma ^{2}}\left( I-\frac{1}{\sigma ^{2}}\Phi
^{T}\Sigma \Phi \right) ,  \nonumber \\
m_{\ast } &=&\mathbf{\phi }\left( \mathbf{q}_{\ast }\right) ^{T}\overline{%
\mathbf{w}},\quad v_{\ast }=\mathbf{\phi }\left( \mathbf{q}_{\ast }\right)
^{T}\Sigma \mathbf{\phi }\left( \mathbf{q}_{\ast }\right) +\sigma ^{2}, 
\nonumber
\end{eqnarray}%
where $I$ is the identity matrix. The latter distribution provides the
predictive mean and the variance. % (note that $v_{\ast }$ is the variance of $%
%y_{\ast }$, which is larger than the variance of $f_{\ast }=f\left( \mathbf{q%
%}_{\ast }\right) $ by $\sigma ^{2}$, see Eq. (\ref{p1})). 
These expressions allow for the computation of the Log-marginal likelihood
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2}\mathbf{y}^{T}\Sigma _{l}^{-1}%
\mathbf{y}-\frac{1}{2}\log \left| \Sigma _{l}\right| -\frac{N}{2}\log \left(
2\pi \right) .  \label{p7}
\end{equation}%
Maximization of this function leads to optimal values of
hyper-parameters, such as $\sigma ^{2}$ and other variables which define $%
\mathbf{\phi }\left( \mathbf{q}\right) $. For example, this can be the
scale, $h$, if the Gaussian functions centered at some points $\mathbf{q}%
_{j}^{\prime }$ (which need not necessarily come from the training set) are
selected as a basis, 
\begin{equation}
\phi _{j}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}%
_{j},h\right) =\exp \left( -\frac{\left\| \mathbf{q-q}_{j}^{\prime }\right\|
^{2}}{h^{2}}\right) ,\quad j=1,...,D,\quad \mathbf{\phi }=\left( \phi
_{1},...,\phi _{D}\right) ^{T}.  \label{p8}
\end{equation}

\subsection{Function-space view}

A Gaussian process % can be defined as a collection of random variables, any
%finite number of which have a joint Gaussian distribution~\cite{rbfgp2}. 
is completely specified by the mean function $ m\left( \mathbf{q}\right) $ 
and the covariance, or kernel, function $k\left( 
\mathbf{q},\mathbf{q}^{\prime }\right) $. %Usually it is assumed that the
%mean is zero, so only $k\left( \mathbf{q},\mathbf{q}^{\prime }\right) $ is
%of concern and there can be a variety of such functions, 
The kernel function is, by definition, symmetric with respect to the arguments.
The regression model described above provides
\begin{eqnarray}
m\left( \mathbf{q}\right)  &=&\mathbb{E}\left[ f\left( \mathbf{q}\right) %
\right] =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{%
w}\right] =0,  \label{p9} \\
k\left( \mathbf{q},\mathbf{q}^{\prime }\right)  &=&\mathbb{E}\left[ f\left( 
\mathbf{q}\right) f\left( \mathbf{q}^{\prime }\right) \right] =\mathbf{\phi }%
\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{ww}^{T}\right] \mathbf{%
\phi }\left( \mathbf{q}^{\prime }\right) =\mathbf{\phi }\left( \mathbf{q}%
\right) ^{T}\mathbb{\Sigma }_{p}\mathbf{\phi }\left( \mathbf{q}^{\prime
}\right) .  \nonumber
\end{eqnarray}

For finite training sets, a $N\times N$ matrix of covariances, 
$K_{mn}=k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right) $ can be
introduced. In the case of Eq. (\ref{p9}) we have%
\begin{equation}
K=\Phi ^{T}\mathcal{\Sigma }_{p}\Phi .  \label{p10}
\end{equation}%
The function-space view provides a solution of the problem with noise in the
form 
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,K+\sigma ^{2}I),\quad y_{\ast }\sim \mathcal{%
N}(m_{\ast },v_{\ast }),  \label{p11} \\
m_{\ast } &=&\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{%
y},\quad v_{\ast }=k\left( \mathbf{q}_{\ast },\mathbf{q}_{\ast }\right) -%
\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{k}_{\ast
}+\sigma ^{2},  \nonumber
\end{eqnarray}%
where $\mathbf{k}_{\ast }$ is a column vector with entries $k\left( \mathbf{q%
}_{n},\mathbf{q}_{\ast }\right) $, $n=1,...,N.$ The marginal likelihood can
be computed using Eq. (\ref{p7}), where matrix $K+\sigma ^{2}I$ should be
used instead of $\Sigma _{l}$.

Note that, in the kernel approach, the predictive mean can be written in the
form similar to that for the weight-space approach (Eqns.~\ref{p4},~\ref{p6})
\begin{equation}
m_{\ast }=f\left( \mathbf{q}_{\ast }\right) =\mathbf{k}_{\ast }^{T}\mathbf{%
\alpha }=\sum_{n=1}^{N}\alpha _{n}k\left( \mathbf{q}_{\ast },\mathbf{q}%
_{n}\right) ,\quad \mathbf{\alpha }=\left( \alpha _{1},...,\alpha
_{N}\right) ^{T}=\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{y}.  \label{p12}
\end{equation}%
The distinctions between the weight and function space approaches are well-recognized~\cite{rbfgp2}, 
but some important points are noted below:
\begin{itemize}
\item The
matrix $\Phi $ can be non-symmetric, while being a covariance matrix $K$
should be symmetric and positive semi-definite. 

\item The number of
basis functions in Eq. (\ref{p12}) is $N$, while the number of basis
functions in Eq. (\ref{p4}) is $D$. 

\item The relation between $K$ and $%
\Phi $ is given by Eq. (\ref{p10}) and the case $K=\Phi $ and $\mathbf{%
\alpha }=\overline{\mathbf{w}}$ realizes only if $D=N$, $\mathbf{q}%
_{n}^{\prime }=\mathbf{q}_{n},$ $\Phi $ is symmetric and and positively
definite, and the covariance matrix for the weigths $\mathcal{\Sigma }%
_{p}=\Phi ^{-1}$. If this is not the case, forms (\ref{p6}) and (\ref{p12})
present expansions over different bases. For example, for Gaussian functions
(\ref{p8}) the function-space view at $\Sigma _{p}=\sigma _{p}^{2}I$
provides according to Eq. (\ref{p10}) the following entries for matrix $%
K=\sigma _{p}^{2}\Phi ^{T}\Phi $ 
\begin{equation}
K_{mn}=\sigma _{p}^{2}\sum_{j=1}^{D}\exp \left( -\frac{\left\| \mathbf{q}%
_{n}-\mathbf{q}_{j}^{\prime }\right\| ^{2}+\left\| \mathbf{q}_{m}-\mathbf{q}%
_{j}^{\prime }\right\| ^{2}}{h^{2}}\right) ,\quad m,n=1,...,N.  \label{p14}
\end{equation}%
So taking limit of this at $\sigma _{p}^{2}\sim 1/D$ and $D\rightarrow
\infty $ we obtain a well known result%
\begin{eqnarray}
k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right)  &=&K_{mn}\sim \int_{\mathbb{R}%
^{d}}\exp \left( -\frac{\left\| \mathbf{q}_{n}-\mathbf{q}^{\prime }\right\|
^{2}+\left\| \mathbf{q}_{m}-\mathbf{q}^{\prime }\right\| ^{2}}{h^{2}}\right)
d\mathbf{q}^{\prime }  \label{p15} \\
&\mathbf{\sim }&\exp \left( -\frac{\left\| \mathbf{q}_{m}-\mathbf{q}%
_{n}\right\| ^{2}}{2h^{2}}\right) ,\quad m,n=1,...,N,  \nonumber
\end{eqnarray}%
which is different from functions (\ref{p8}) as the Gaussians in kernel $%
k\left( \mathbf{q},\mathbf{q}^{\prime }\right) $ have larger scale, $2^{1/2}h
$, the functions $\phi _{j}\left( \mathbf{q}\right) $. 
\end{itemize}

%The difference
%between the weight and function space view for the Gaussian basis function
%sometimes is missed by the researchers, as soon as parameter $h$ is selected
%from optimization problem (maximization of the marginal likelyhood).

\textcolor{red}{
This section is good, but may have to cut the text a bit (can move some things to appendix)
Also need a better end the section
}



==> gp_newNG.tex <==

\section{Preliminaries of GP regression}
In this section, a brief review of standard GP regression is presented. While a
detailed review can be found in the excellent book by Rasmussen~\cite{rbfgp2},
the description and notations below provide the necessary context for the development
of the multiscale algorithm proposed in this paper. 

We consider the finite dimensional weight-space view
and the infinite dimensional function-space view as in Rasmussen~\cite{rbfgp2}. 
Given a
training set $\mathcal{D}$ of $N$ observations, $\mathcal{D}=\left\{ \left( 
\mathbf{q}_{n},y_{n}\right)~|~n=1,...,N\right\} $, where $%
\mathbf{q}_{n}\in \mathbb{R}^{d}$ is an input vector and $y$ is a scalar
output, the goal is to obtain the predictive mean, $%
m_{\ast }$, and variance, $v_{\ast }$, at an arbitrary test point $\mathbf{q}%
_{\ast }\in \mathbb{R}^{d}$. Training inputs are collected in the design
matrix $Q\in \mathbb{R}^{d\times N}$, and the outputs form the vector $\mathbf{%
y\in }$ $\mathbb{R}^{N}$. Furthermore, it is assumed that%
\begin{equation}
y=f\left( \mathbf{q}\right) +\epsilon ,\quad \epsilon \sim \mathcal{N}%
(0,\sigma ^{2}),  \label{p1}
\end{equation}%
where $\epsilon $ is Gaussian noise with zero mean and variance $\sigma ^{2}$.

\subsection{Weight-space view}

The standard linear regression model presents $f\left( \mathbf{q}\right) $
in Eq. (\ref{p1}) as

\begin{equation}
f\left( \mathbf{q}\right) =\mathbf{q}^{T}\mathbf{w,}  \label{p2}
\end{equation}%
where $\mathbf{w\in }$ $\mathbb{R}^{d}$ is the vector of weights. 
%In Bayesian analysis, one
%specifies a prior and computes the posterior distribution.  Particularly, 
If the prior distribution of the weights is  a multivariate Gaussian with zero
mean and covariance matrix $\Sigma _{p}$, then the posterior distribution is
also a multivariate Gaussian with mean $\overline{\mathbf{w}}$ and covariance
matrix $\Sigma $: 
\begin{equation}
\overline{\mathbf{w}}=\frac{1}{\sigma ^{2}}\Sigma Q\mathbf{y,\quad }\Sigma
^{-1}=\frac{1}{\sigma ^{2}}QQ^{T}+\Sigma _{p}^{-1}.  \label{p3}
\end{equation}

For low dimensionality $d$ of the inputs, linear regression
cannot satisfy a variety of dependencies encountered in practice. Therefore, the input is mapped into a high-dimensional feature space $\mathbb{R}%
^{D},$ $D>d$, and the linear regression model is applied in this
space. To avoid any confusion with the original feature space $\mathbb{R}^{d}
$, this space will be referred to as the ``extended feature space'' and its
dimensionality can be referred to as the ``size'' of the system. Denoting the mapping function $%
\mathbf{\phi }\left( \mathbf{q}\right) $, $\mathbf{\phi }:\mathbb{R}%
^{d}\rightarrow \mathbb{R}^{D}$ we have%
\begin{equation}
f\left( \mathbf{q}\right) =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}%
\mathbf{w=}\sum_{j=1}^{D}w_{j}\phi _{j}\left( \mathbf{q}\right) \mathbf{%
,\quad w}=\left( w_{1},...,w_{D}\right) \in \mathbb{R}^{D}.  \label{p4}
\end{equation}%
%The analysis in this case is similar to that for the linear regression.
%Particularly, 
The covariance matrices $\Sigma _{p}$ and $\Sigma $ have sizes 
$D\times D$ instead of $d\times d$. The design matrix $Q$ should be
replaced by matrix $\Phi \in \mathbb{R}^{D\times N}$, whose columns are $\mathbf{%
\phi }\left( \mathbf{q}_{n}\right) $ instead of $\mathbf{q}_{n}$, $n=1,...,N.
$ The predictive mean and the covariance matrix can then be computed as%
\begin{equation}
\overline{\mathbf{w}}=\frac{1}{\sigma ^{2}}\Sigma \Phi \mathbf{y,\quad }%
\Sigma ^{-1}=\frac{1}{\sigma ^{2}}\Phi \Phi ^{T}+\Sigma _{p}^{-1}.
\label{p5}
\end{equation}%
The Bayesian formalism provides Gaussian distributions for the training
outputs and for the predictive mean $m_{\ast }$ and variance $v_{\ast }$.%
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,\Sigma _{l}),\quad y_{\ast }\sim \mathcal{N}%
(m_{\ast },v_{\ast }),  \label{p6} \\
\Sigma _{l}^{-1} &=&\frac{1}{\sigma ^{2}}\left( I-\frac{1}{\sigma ^{2}}\Phi
^{T}\Sigma \Phi \right) ,  \nonumber \\
m_{\ast } &=&\mathbf{\phi }\left( \mathbf{q}_{\ast }\right) ^{T}\overline{%
\mathbf{w}},\quad v_{\ast }=\mathbf{\phi }\left( \mathbf{q}_{\ast }\right)
^{T}\Sigma \mathbf{\phi }\left( \mathbf{q}_{\ast }\right) +\sigma ^{2}, 
\nonumber
\end{eqnarray}%
where $I$ is the identity matrix. %The last equation above provides the
%predictive mean and the variance. % (note that $v_{\ast }$ is the variance of $%
%y_{\ast }$, which is larger than the variance of $f_{\ast }=f\left( \mathbf{q%
%}_{\ast }\right) $ by $\sigma ^{2}$, see Eq. (\ref{p1})). 
These expressions allow for the computation of the log-marginal likelihood (LML),
\begin{equation}
\log p\left( \mathbf{y}|Q\right) =-\frac{1}{2}\mathbf{y}^{T}\Sigma _{l}^{-1}%
\mathbf{y}-\frac{1}{2}\log \left| \Sigma _{l}\right| -\frac{N}{2}\log \left(
2\pi \right) .  \label{p7}
\end{equation}%
Maximization of this function leads to optimal values of
hyper-parameters such as $\sigma ^{2}$ and other variables that define $%
\mathbf{\phi }\left( \mathbf{q}\right) $. For example, this can be the
scale, $h$, if Gaussian functions centered at some points $\mathbf{q}%
_{j}^{\prime }$ (which need not necessarily come from the training set) are
selected as a basis: 
\begin{equation}
\phi _{j}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}%
_{j},h\right) =\exp \left( -\frac{\left\| \mathbf{q-q}_{j}^{\prime }\right\|
^{2}}{h^{2}}\right) ,\quad j=1,...,D,\quad \mathbf{\phi }=\left( \phi
_{1},...,\phi _{D}\right) ^{T}.  \label{p8}
\end{equation}

\subsection{Function-space view}

A Gaussian process % can be defined as a collection of random variables, any
%finite number of which have a joint Gaussian distribution~\cite{rbfgp2}. 
is completely specified by the mean function $ m\left( \mathbf{q}\right) $ 
and the covariance, or kernel, function $k\left( 
\mathbf{q},\mathbf{q}^{\prime }\right) $. %Usually it is assumed that the
%mean is zero, so only $k\left( \mathbf{q},\mathbf{q}^{\prime }\right) $ is
%of concern and there can be a variety of such functions, 
The kernel function is, by definition, symmetric with respect to the arguments.
The regression model described above provides
\begin{eqnarray}
m\left( \mathbf{q}\right)  &=&\mathbb{E}\left[ f\left( \mathbf{q}\right) %
\right] =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{%
w}\right] =0,  \label{p9} \\
k\left( \mathbf{q},\mathbf{q}^{\prime }\right)  &=&\mathbb{E}\left[ f\left( 
\mathbf{q}\right) f\left( \mathbf{q}^{\prime }\right) \right] =\mathbf{\phi }%
\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{ww}^{T}\right] \mathbf{%
\phi }\left( \mathbf{q}^{\prime }\right) =\mathbf{\phi }\left( \mathbf{q}%
\right) ^{T}\boldsymbol{\Sigma}_{p}\mathbf{\phi }\left( \mathbf{q}^{\prime
}\right) .  \nonumber
\end{eqnarray}

For finite training sets, a $N\times N$ matrix of covariances, 
$K_{mn}=k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right) $ can be
introduced. In the case of Eq. (\ref{p9}), we have%
\begin{equation}
K=\Phi ^{T}\boldsymbol{\Sigma}_{p}\Phi .  \label{p10}
\end{equation}%
The function-space view provides a solution of the problem in the
form 
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,K+\sigma ^{2}I),\quad y_{\ast }\sim \mathcal{%
N}(m_{\ast },v_{\ast }),  \label{p11} \\
m_{\ast } &=&\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{%
y},\quad v_{\ast }=k\left( \mathbf{q}_{\ast },\mathbf{q}_{\ast }\right) -%
\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{k}_{\ast
}+\sigma ^{2},  \nonumber
\end{eqnarray}%
where $\mathbf{k}_{\ast }$ is a column vector with entries $k\left( \mathbf{q%
}_{n},\mathbf{q}_{\ast }\right) $, $n=1,...,N.$ The marginal likelihood can
be computed using Eq. (\ref{p7}), where the matrix $K+\sigma ^{2}I$ is
used in place of $\Sigma _{l}$.

Note that, in the kernel approach, the predictive mean can be written in a
form similar to that in the weight-space approach (Eqns.~\ref{p4},~\ref{p6})
\begin{equation}
m_{\ast }=f\left( \mathbf{q}_{\ast }\right) =\mathbf{k}_{\ast }^{T}\mathbf{%
\alpha }=\sum_{n=1}^{N}\alpha _{n}k\left( \mathbf{q}_{\ast },\mathbf{q}%
_{n}\right) ,\quad \mathbf{\alpha }=\left( \alpha _{1},...,\alpha
_{N}\right) ^{T}=\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{y}.  \label{p12}
\end{equation}%
The distinction between the weight- and function-space approaches has been
 documented~\cite{rbfgp2}, 
but some important points are noted below:
\begin{itemize}
\item The
matrix $\Phi $ can be non-symmetric, while the covariance matrix $K$
should be symmetric and positive semi-definite. 

\item The number of
basis functions in Eq. (\ref{p12}) is $N$, while the number of basis
functions in Eq. (\ref{p4}) is $D$. 

\item The relationship between $K$ and $%
\Phi $ is given by Eq. (\ref{p10}), and the case $K=\Phi $ and $\mathbf{%
\alpha }=\overline{\mathbf{w}}$ is realized only if $D=N$, $\mathbf{q}%
_{n}^{\prime }=\mathbf{q}_{n},$ $\Phi $ is symmetric and positive
definite, and the covariance matrix for the weights $\boldsymbol{\Sigma}%
_{p}=\Phi ^{-1}$. If this is not the case, forms (\ref{p6}) and (\ref{p12})
present expansions over different bases. For example, for Gaussian functions
(\ref{p8}), the function-space view with $\Sigma _{p}=\sigma _{p}^{2}I$
provides, according to Eq. (\ref{p10}), the following entries for matrix $%
K=\sigma _{p}^{2}\Phi ^{T}\Phi $:
\begin{equation}
K_{mn}=\sigma _{p}^{2}\sum_{j=1}^{D}\exp \left( -\frac{\left\| \mathbf{q}%
_{n}-\mathbf{q}_{j}^{\prime }\right\| ^{2}+\left\| \mathbf{q}_{m}-\mathbf{q}%
_{j}^{\prime }\right\| ^{2}}{h^{2}}\right) ,\quad m,n=1,...,N.  \label{p14}
\end{equation}%

Taking the limit of this at $\sigma _{p}^{2}\sim 1/D$ and $D\rightarrow
\infty $, we obtain a well-known result:%
\begin{eqnarray}
k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right)  &=&K_{mn}\sim \int_{\mathbb{R}%
^{d}}\exp \left( -\frac{\left\| \mathbf{q}_{n}-\mathbf{q}^{\prime }\right\|
^{2}+\left\| \mathbf{q}_{m}-\mathbf{q}^{\prime }\right\| ^{2}}{h^{2}}\right)
d\mathbf{q}^{\prime }  \label{p15} \\
&\mathbf{\sim }&\exp \left( -\frac{\left\| \mathbf{q}_{m}-\mathbf{q}%
_{n}\right\| ^{2}}{2h^{2}}\right) ,\quad m,n=1,...,N,  \nonumber
\end{eqnarray}%
which is different from Eq. (\ref{p8}) because the Gaussians in kernel $%
k\left( \mathbf{q},\mathbf{q}^{\prime }\right) $ have larger scales, $2^{1/2}h
$, than the functions $\phi _{j}\left( \mathbf{q}\right) $. 
\end{itemize}

%The difference
%between the weight and function space view for the Gaussian basis function
%sometimes is missed by the researchers, as soon as parameter $h$ is selected
%from optimization problem (maximization of the marginal likelyhood).

While the weight-space and the kernel approaches have similarities, the
complexity of these algorithms can be different in practice and the optimization 
of the hyper-parameters may also be different.


==> gp_revised_NG_text.tex <==

\section{Preliminaries of GP regression}

In this section, a brief review of standard GP regression is presented.
While a detailed review can be found in the excellent book by Rasmussen~\cite%
{rbfgp2}, the description and notations below provide the necessary context
for the development of the multiscale algorithm proposed in this paper.

We consider the finite dimensional weight-space view and the infinite
dimensional function-space view as in Rasmussen~\cite{rbfgp2}. Given a
training set $\mathcal{D}$ of $N$ observations, $\mathcal{D}=\left\{ \left( 
\mathbf{q}_{n},y_{n}\right)~|~n=1,...,N\right\} $, where $\mathbf{q}_{n}\in 
\mathbb{R}^{d}$ is an input vector and $y$ is a scalar output, the goal is
to obtain the predictive mean, $m_{\ast }$, and variance, $v_{\ast }$, at an
arbitrary test point $\mathbf{q}_{\ast }\in \mathbb{R}^{d}$. Training inputs
are collected in the design matrix $Q\in \mathbb{R}^{d\times N}$, and the
outputs form the vector $\mathbf{y\in }$ $\mathbb{R}^{N}$. Furthermore, it
is assumed that%
\begin{equation}
y=f\left( \mathbf{q}\right) +\epsilon ,\quad \epsilon \sim \mathcal{N}%
(0,\sigma ^{2}),  \label{p1}
\end{equation}%
where $\epsilon $ is Gaussian noise with zero mean and variance $\sigma ^{2}$%
.

For low dimensionality $d$ of the inputs, linear regression cannot satisfy a
variety of dependencies encountered in practice. Therefore, the input is
mapped into a high-dimensional feature space $\mathbb{R}^{D},$ $D>d$, and
the linear regression model is applied in this space. To avoid any confusion
with the original feature space $\mathbb{R}^{d}$, this space will be
referred to as the ``extended feature space'' and its dimensionality can be
referred to as the ``size'' of the system. Denoting the mapping function $%
\mathbf{\phi }\left( \mathbf{q}\right) $, $\mathbf{\phi }:\mathbb{R}%
^{d}\rightarrow \mathbb{R}^{D}$ we have%
\begin{equation}
f\left( \mathbf{q}\right) =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}%
\mathbf{w=}\sum_{j=1}^{D}w_{j}\phi _{j}\left( \mathbf{q}\right) \mathbf{%
,\quad w}=\left( w_{1},...,w_{D}\right) \in \mathbb{R}^{D}.  \label{p4}
\end{equation}%
The predictive mean and the covariance matrix can then be computed as%
\begin{equation}
\overline{\mathbf{w}}=\frac{1}{\sigma ^{2}}\Sigma \Phi \mathbf{y,\quad }%
\Sigma ^{-1}=\frac{1}{\sigma ^{2}}\Phi \Phi ^{T}+\Sigma _{p}^{-1}.
\label{p5}
\end{equation}%
The Bayesian formalism provides Gaussian distributions for the training
outputs and for the predictive mean $m_{\ast }$ and variance $v_{\ast }$.%
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,\Sigma _{l}),\quad y_{\ast }\sim \mathcal{N}%
(m_{\ast },v_{\ast }),  \label{p6} \\
\Sigma _{l}^{-1} &=&\frac{1}{\sigma ^{2}}\left( I-\frac{1}{\sigma ^{2}}\Phi
^{T}\Sigma \Phi \right) ,  \nonumber \\
m_{\ast } &=&\mathbf{\phi }\left( \mathbf{q}_{\ast }\right) ^{T}\overline{%
\mathbf{w}},\quad v_{\ast }=\mathbf{\phi }\left( \mathbf{q}_{\ast }\right)
^{T}\Sigma \mathbf{\phi }\left( \mathbf{q}_{\ast }\right) +\sigma ^{2}, 
\nonumber
\end{eqnarray}%
where $I$ is the identity matrix. These expressions allow for the
computation of the log-marginal likelihood (LML), 
\begin{equation}
\log p\left( \mathbf{y}|Q\right) =-\frac{1}{2}\mathbf{y}^{T}\Sigma _{l}^{-1}%
\mathbf{y}-\frac{1}{2}\log \left| \Sigma _{l}\right| -\frac{N}{2}\log \left(
2\pi \right) .  \label{p7}
\end{equation}%
Maximization of this function leads to optimal values of hyper-parameters
such as $\sigma ^{2}$ and other variables that define $\mathbf{\phi }\left( 
\mathbf{q}\right) $. 

A Gaussian process is completely specified by the mean function $m\left( 
\mathbf{q}\right) $ and the covariance, or kernel, function $k\left( \mathbf{%
q},\mathbf{q}^{\prime }\right) $. The regression model described above
provides 
\begin{eqnarray}
m\left( \mathbf{q}\right)  &=&\mathbb{E}\left[ f\left( \mathbf{q}\right) %
\right] =\mathbf{\phi }\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{%
w}\right] =0,  \label{p9} \\
k\left( \mathbf{q},\mathbf{q}^{\prime }\right)  &=&\mathbb{E}\left[ f\left( 
\mathbf{q}\right) f\left( \mathbf{q}^{\prime }\right) \right] =\mathbf{\phi }%
\left( \mathbf{q}\right) ^{T}\mathbb{E}\left[ \mathbf{ww}^{T}\right] \mathbf{%
\phi }\left( \mathbf{q}^{\prime }\right) =\mathbf{\phi }\left( \mathbf{q}%
\right) ^{T}\boldsymbol{\Sigma}_{p}\mathbf{\phi }\left( \mathbf{q}^{\prime
}\right) .  \nonumber
\end{eqnarray}

For finite training sets, a $N\times N$ matrix of covariances, $%
K_{mn}=k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right) $ can be introduced. In
the case of Eq. (\ref{p9}), we have%
\begin{equation}
K=\Phi ^{T}\boldsymbol{\Sigma}_{p}\Phi .  \label{p10}
\end{equation}%
The function-space view provides a solution of the problem in the form 
\begin{eqnarray}
\mathbf{y} &\sim &\mathcal{N}(0,K+\sigma ^{2}I),\quad y_{\ast }\sim \mathcal{%
N}(m_{\ast },v_{\ast }),  \label{p11} \\
m_{\ast } &=&\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{%
y},\quad v_{\ast }=k\left( \mathbf{q}_{\ast },\mathbf{q}_{\ast }\right) -%
\mathbf{k}_{\ast }^{T}\left( K+\sigma ^{2}I\right) ^{-1}\mathbf{k}_{\ast
}+\sigma ^{2},  \nonumber
\end{eqnarray}%
where $\mathbf{k}_{\ast }$ is a column vector with entries $k\left( \mathbf{q%
}_{n},\mathbf{q}_{\ast }\right) $, $n=1,...,N.$ The marginal likelihood can
be computed using Eq. (\ref{p7}), where the matrix $K+\sigma ^{2}I$ is used
in place of $\Sigma _{l}$.



==> introduction_3old.tex <==
\section{Introduction}

The rapid growth in computing power has resulted in the generation of massive amounts of highly resolved datasets in many field of science and engineering. 
Against this backdrop, machine learning (ML)  is becoming a widely used tool to identify patterns and functional relationships to enable improved understanding 
of the underlying physical phenomena, to improve predictive models and in applications such as controlling complex systems. In this work, we are specifically
interested in regression techniques that fall under the class of supervised learning methods.
Gaussian process (GP) regression is one such popular ML technique that is capable of providing accurate predictions of the mean and variance of functional 
outputs. 

A major disadvantage to GPs, however, is that they can be highly expensive to train, and slow to evaluate. 
\textcolor{red}{
	expand a bit more, talk about sparsity, high dimensions, etc.
}
The computational complexity of GPs at the training stage is tied to the kernel inversion and the computation of the 
Log-marginal likelihood. For example,
an algorithm based on the Cholesky decomposition is one well-known approach\cite{chol}. The computational complexity of Cholesky decomposition for a 
problem with $N$ training points is $O\left( N^{3}\right) $. Even if this cost can be reduced using, for instance, 
iterative methods~\cite{gumerov_iterative}, the
computation of the predictive mean and variance at $M$ test points still scale as $O\left(N M\right) $, 
and $O\left(N^{2} M\right) $, respectively.
The evaluation (or testing time) could be of greater significance than the training time if GP evaluations are made frequently during a computation process. 
Such a requirement can occur in a scientific computing setting~\cite{our_own_aiaa_paper,our_own_jcp_paper} when large scale GP evaluations are performed
every time-step or iteration of the solver.  Reducing both the training and evaluation costs, while preserving
the accuracy of GP regression is the goal of the current work.

Much effort has been devoted to the construction of algorithms of reduced complexity. Among these is the family of methods of sparse Gaussian process regression. These methods seek to strategically reduce the size of the training set or find appropriate sparse representations of the correlation matrix $\mb{\Phi}$ through the use of induced variables. Descriptions for several methods of this family are provided by Qui{\~n}onero-Candela et. al. \cite{quinonero2005}, who define induced variables $\mb{U}\in \mathbb{R}^{N^\prime \times d}$, $\mb{V}\in \mathbb{R}^{N^\prime}$ such that the prediction of a function $f$ is given by

\begin{equation}
p(f|\mb{U}) \sim \mc{N}(\underline{\phi}_u^T\mb{\Phi}_u^{-1}\mb{V}, 1+\lambda-\underline{\phi}_u^T\mb{\Phi}_u^{-1}
\underline{\phi}_u)
\end{equation}

where $\underline{\phi}_u$ is a vector whose elements are $\phi(\mb{u}_i,\mb{q}_{\mr{test}})$, and $\mb{\Phi}_u(m,n) = \phi(\mathbf{u}_m,\mathbf{u}_n)$. From this, it is evident that if $N^\prime<N$, the matrix inversion will be less costly to perform. 

It can be difficult to decide upon an optimal algorithm to determine the induced variables that represent the training set best, and these algorithms introduce additional computational cost. The most basic method to select them is to randomly select a fraction of points and define them as the new training set, i.e. choosing $(\mb{U},\mb{V})$ from $(\mb{Q}_{\mr{train}},\mb{Y}_{\mr{train}})$. Seeger \cite{seeger2003}, Smola \cite{smola2001}, and others have developed  selection methods that provide better test results compared to random selection. These methods often depend on optimising modified likelihoods based on $(\mb{U},\mb{V})$ or on approximating the true LML \cite{titsias2009}. Methods that introduce new induced variables instead of choosing from training points can involve solving optimisation problems, again requiring the user to consider the additional computational resources required. 

In addition to choosing the inducing variables, one may also change the form of the covariance matrix from $\phi$ to $\phi'$, where
\[\phi'(\mb{q}_m,\mb{q}_n) = \phi(\mb{q}_m,\mb{U})\mb{\Phi}_u^{-1}\phi(\mb{q}_n,\mb{U})^T\]
Unlike in the case where only a subset of training data is used, all training points are considered, and the matrices are only of rank $M$. There are many variations on this type of manipulation of the covariance. Alternatively, one can approximate $\mb{\Phi}$ directly by taking random samples of the kernel, which is described in \cite{recht2007}. Altering the correlation matrix can cause various undesirable behaviours when computing the test variance, since some matrices no longer correspond to a Gaussian process mathematically. 

Other methods of speeding up GP regression focus on dividing the training set into smaller sets of more manageable size. Snelson and Ghahramani \cite{snelson2007local} employ a local GP consisting of points in the neighbourhood of the test point in addition to a simplified global estimate to improve test results. Urtasun and Darrell \cite{urtasun2008} use the local GP directly, without the induced variables. However, this means test points must either be assigned to a precomputed neighbourhood of training points, as in the former publication, or points must be found on-line for every test point, as in the latter. Both can be quite expensive depending on training set size, though massive parallelisation may mitigate the cost in some aspects \cite{keane2002} \cite{weiss2014}.
\textcolor{red}{
You've spoken about speed, but what about efforts to address accuracy?
}

Overall, the changes that need to be made to the GP depend upon the resources at hand and the problem that is being addressed. For on-line applications, the main necessity is test speed. However, it would be unwise to ignore training requirements even though training takes place off-line, since the input space is large and new training data may have to be incorporated relatively quickly; time and memory usage must both be taken into account. In this work, a new alteration to GP that could address these specific areas is introduced.
\textcolor{red}{
\begin{itemize}
\item be more specific about contributions of the paper.
\item this is a long paper, so need a outline of what each section is trying to do
\end{itemize}
}




==> introduction_Orig.tex <==
\section{Introduction}
%With the rising availability of raw computational data and computing power, many novel approaches in turbulence modelling are becoming possible, even popular. One such approach, broadly termed data-driven modelling, leverages large databases of various flows in order to generate optimal models through machine learning (ML). This method aims to improve existing models by discovering relationships between flow variables that may not be immediately obvious to the traditional analytical approach. In addition to improving the accuracy of the output, certain machine learning techniques are also capable of providing estimates of the accuracy. When coupled with the traditional turbulence model, it may be able to provide useful information on the uncertainty of the process as a whole.

Machine learning is the process of deriving patterns from data, patterns which may then be used to for making predictions. In order to maximise the usefulness of available data, the ML method should be able to work with very large, very multi-dimensional input data sets. This is because the practical applications that would benefit from machine learning are typically complex and indeed necessitate the usage of such datasets rather than more direct models to achieve desired results. Subsets of the data can be used as training sets to predict observations, and the quality of these predictions are estimated by directly using other subsets as test points, or by taking probabilistic approaches. In machine learning, this is termed supervised learning, because the goal is to map an input to an output, and is in particular referred to as regression, because the outputs are variables and not group identifiers. 

Gaussian process (GP) regression is a machine learning technique that by its nature is capable of generating uncertainty bounds on the output. This is useful for many applications. Specifically, for simulation-type applications, the uncertainty of the learning process can be carried through the simulation and thus lead to uncertainty estimates on the output quantities of interest. In other words, in being passed through another process, the estimate is one step removed from the final product. Since it is integrated early on, the uncertainty will incorporate the effects of the form of the base model and therefore hopefully prove to be of use to engineers. However, the main disadvantage to GPs is that they can be slow to train, that is, to set up using the training database of points, and also slow to evaluate. As will be shown later, this is because their evaluation speed scales linearly with the number of test points. This is undesirable in practice because typically, the model will need to be evaluated frequently. High evaluation cost can dramatically slow the workflow and negate any advantages gained over using simpler, faster models.

Another challenge inherent in the problem is the high dimensionality of the input space. This is because it is usually necessary to use many input variables in order to describe the complex behaviour of the output variable. The more variables used as inputs, the more sparse the input space becomes, and the more data required to span the input space in order to avoid extrapolation, a task at which ML does not typically perform well. 

This work presents a new approach, multiscale Gaussian process (MGP) regression, based on ordinary GP regression. The key goal of this new method is to improve the speed of GPs while preserving their accuracy, which is derived from using many training points that span the input space. It is hoped that MGP will increase the feasibility of using data-driven models under limited resources. To do this, MGP makes judicious selections from the input data and reduces the effective size of the dataset while preserving necessary information by separating the data into scales. The process also leads to better prediction of data that forms clusters in input space, which is likely the case for high-dimensional input spaces.

In the next section, the basics of Gaussian processes are presented. Following this, the new method, MGP, will be explained. Both will then be applied in numerical examples. 

\textcolor{red}{
Intro section
\begin{itemize}
\item This has not been altered since first or second draft
\end{itemize}
}

==> mgp_new.tex <==
\section{Multiscale sparse GP regression}
As stated earlier, the goal of the proposed GP-based regression process is to decrease the order of complexity of both training and testing 
and to make the prediction more robust for datasets that have a highly irregular distribution of features.
%We start with the selection of multiple values
%of the scale parameter $h$.  
%In this case, the derivation of a compact kernel or
%covariance function in infinite-dimensional feature spaces is a
%non-trivial task because of the dependence on the apriori unknown continuous scale
%distribution (in integral (\ref{p15}) $h$ should be treated as an arbitrary
%function of $\mathbf{q}^{\prime }$ in which case a closed analytic firm is
%possible only for the cases of special assumptions. On the other hand, both
%views described above can be applied to the treatment of the problem for
%finite dimensional feature spaces.

We begin with a generalization of basis functions (\ref{p8}),%
\begin{equation}
\phi _{j}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}_{j}^{\prime
},h_{j}\right) =\exp \left( -\frac{\left\| \mathbf{q-q}_{j}^{\prime
}\right\| ^{2}}{h_{j}^{2}}\right) ,\quad j=1,...,D,\quad \mathbf{\phi }%
=\left( \phi _{1},...,\phi _{D}\right) ^{T},  \label{m1}
\end{equation}%
where each function is characterized not only by its center $\mathbf{q}_{j}$%
, but also by a scale $h_{j}$. The need
for such a generalization may arise from the underlying physics (e.g. particle
density estimation) or just to the substantial non-uniformity of the
input data distribution, which could for instance, demand smaller scales in denser
regions.

We note that the the matrix $\Phi \Phi ^{T}$ (which is required for the
computation of covariance matrix $\Sigma $ in Eq. (\ref{p5}) and the kernel matrix $K$ in Eq. (\ref{p10}) ).%
is given by
\begin{eqnarray}
\left( \Phi \Phi ^{T}\right) _{ij} &=&\sum_{n=1}^{N}\phi _{i}\left( \mathbf{q%
}_{n}\right) \phi _{j}\left( \mathbf{q}_{n}\right)   \label{m2} \\
&=&\sum_{n=1}^{N}\exp \left( -\frac{\left\| \mathbf{q}_{n}-\mathbf{q}%
_{i}^{\prime }\right\| ^{2}}{h_{i}^{2}}-\frac{\left\| \mathbf{q}_{n}-\mathbf{%
q}_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad i,j=1,...,D, 
\nonumber
\end{eqnarray}%
\begin{eqnarray}
k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right)  &=&K_{mn}=\sigma
_{p}^{2}\sum_{j=1}^{D}\phi _{j}\left( \mathbf{q}_{m}\right) \phi _{j}\left( 
\mathbf{q}_{n}\right)   \label{m3} \\
&=&\sigma _{p}^{2}\sum_{j=1}^{D}\exp \left( -\frac{\left\| \mathbf{q}_{m}-%
\mathbf{q}_{j}^{\prime }\right\| ^{2}+\left\| \mathbf{q}_{n}-\mathbf{q}%
_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad m,n=1,...,N.  \nonumber
\end{eqnarray}

\subsection{Sparse representations}

While there are $N$ training points available and maximum information
can be obtained when the dimensionality of the feature space $D=N$, we will
search for subsets of these points, which provide lower dimensionality of
the feature space, $D<N$. 
%The rationale for this comes from observation,
%that in interpolation problems basis functions typically can be expanded
%over the other basis functions with a sufficient accuracy (prescribed,
%determined by the noise level, or other practical reasons). This is a
%demonstration of the ill-posedness of the problem, which in the GP
%regression approach, in fact, is regularized similarly to the least square
%solution for noisy data (Tikhonov regularization [\textbf{REFERENCE}]).
The dimensionality of the feature space is related to the accuracy of the low
rank approximation of matrix $\Phi $ built on the entire training set, {\em i.e.}
for the case $D=N$. Assume for a moment that we have a single scale, $%
h_{1}=...=h_{N}=h.$ It can be selected to be very small, say smaller than
the minimal distance between the training points, then the matrix $\Phi $
will have a low condition number, the problem will be well-posed, but the
marginal likelihood will be very low. On the other end, if $h$ is
substantially larger than the maximum distance between the training points
the problem will be ill-posed and the marignial likelihood will be also low.
The optima should lie somewhere in between, but if the solution is not
sensitive to the removal of a few training points, a good low-rank approximation can be sought.

The fact that the $N\times N$ matrix $\Phi $ can be well approximated with a
matrix of rank $r<N$, means that $N-r$ rows or columns of this matrix can be
expressed as a linear combination of the other rows or columns with a
relatively small error $\epsilon ^{\prime }$. Assuming that $r$ locations (or centers) of the radial basis functions (or Gaussians) are given and
denoting such centers by $\mathbf{q}_{j}^{\prime }$, $j=1,...,r$, we have
\begin{equation}
\phi _{n}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}%
_{n},h_{n}\right) =\sum_{j=1}^{r}\eta _{nj}\phi _{j}\left( \mathbf{q}\right)
+\epsilon _{n}^{\prime },\quad \mathbf{q}_{j}^{/}\in \mathbb{Q}^{\prime }%
\mathbb{\subset Q}\text{,\quad }n=1,...,N,  \label{m4}
\end{equation}%
where $\eta _{nj}$ are coefficients to be determined. Hence, output (\ref{p1}), where $f$
is expanded as (\ref{p4}) with $D=N$ can be written as%
\begin{eqnarray}
y\left( \mathbf{q}\right)  &=&\sum_{n=1}^{N}w_{n}\phi _{n}\left( \mathbf{q}%
\right) +\epsilon =\sum_{j=1}^{r}w_{j}^{\prime }\phi _{j}\left( \mathbf{q}%
\right) +\epsilon +\epsilon ^{\prime }\mathbf{,}  \label{m5} \\
w_{j}^{\prime } &=&\sum_{n=1}^{N}w_{n}\eta _{nj},\quad \epsilon ^{\prime
}=\sum_{n=1}^{N}w_{n}\epsilon _{n}^{\prime }.  \nonumber
\end{eqnarray}%
This shows that if $\epsilon ^{\prime }$ is lower or comparable with noise $%
\epsilon $, then a reduced basis can be used and one can simply set the
dimensionality of the feature space to be the rank of the low rank
approximation, $D=r$, and coefficients $w_{j}^{\prime }$ can be determined
by solving a $D\times D$, instead of a $N\times N$ problem.

\subsection{Representative training subsets}

Let us consider now the problem of determination of the centers of the basis
functions and scales $h_{j}$. Note that in a single-scale process $h$ is
not known and is determined together with other hyper-parameters by maximizing the LML~\ref{eqn??}.
 If each data-point is assigned a different scale, then the optimization problem will become unwieldy as
$D$ hyperparameters will have to be determined. Some compromises can be made here, where
Instead, we use several scales $h_{1},...,h_{S}$. In the
limit $S=1$ we have a single scale model, while at $S=D$ we prescribe a
scale to each training point. To reduce the number of scales, while
providing a broad spectrum of scales, we propose to consider hierarchical
scales, e.g. $h_{s}=h_{1}\beta ^{s-1}$, $s=1,...,S$, where $h_{1}$ is of the
order of the size of the computational domain and $\beta <1$ is some
dimensionless parameter controlling the scale reduction.

While there exist several randomization-based strategies to obtain a low rank representation
by choosing $D $ representative input points [\textbf{REFERENCES}], we propose a
more regular, structured approach.  For a given scale $h$, we can specify some distance $a=\gamma h$, where $%
\gamma <1$ is chosen such that,
\begin{itemize}
\item The basis points are located further than $a$,
and, on the other hand, they are not too far from each other, so the distance
from any other input point to the basis point is less than $a$. Such a
construction provides, first, a more or less uniform coverage of the entire
training set with $d$-dimensional balls of radius $a$.

\item The number of such balls is - in some sense - optimal. Note that smaller $\gamma $ results in
smaller errors $\epsilon _{n}^{\prime }$ and $\epsilon ^{\prime }$ and
larger $r$ in Eqs (\ref{m4}) and (\ref{m5}). If $\gamma <h/a_{\min }$, where 
$a_{\min }$ is the minimal distance between the points in the training set,
then $\epsilon^{\prime }=0$, $r=D=N$, which corresponds to a full rank
representation.
\end{itemize}

The the problem of constructing an optimal set as 
described above is computational NP-hard problem. However, approximate solutions 
can be obtained with a modification of the well-known $k$-center algorithm~\cite{kcenter}.
In computational geometry problems, the $k$-center
algorithm partitions a domain in $d$-dimensional space to a prescribed
number, $k$, of clusters. The the present problem, however, the number of clusters is
unknown, but the distance parameter $a$ is prescribed. Thus the number of
centers depends on the input point distribution and can be determined after the
algorithm is executed. Since only the cluster centers are required for the
present problem, the following algorithm is used 
\vspace{0.3cm}

\begin{mdframed}
\center{\bf Algorithm \#1: Determination of cluster centers and k}
\vspace{0.3cm}

{\bf Input:} set of training points $\mathbb{Q=}\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, max cluster radius $a$. 


\begin{enumerate}
\item Define $\mathbb{R}_{0}=\mathbb{Q}$ and set $k=0$;

\item Do steps 3 to 6 while $\mathbb{R}_{k}\neq \emptyset ;$

\item $k=k+1;$

\item Assign $\mathbf{q}_{k}^{\prime }=\mathbf{q}_{j}\in $ $\mathbb{R}_{k-1}$
(where $\mathbf{q}_{j}$ is a random point from set $\mathbb{R}_{k-1}$)

\item Find all points $\mathbf{q}_{ki}\in \mathbb{R}_{k-1}$, such that $%
\left| \mathbf{q}_{ki}-\mathbf{q}_{k}^{\prime }\right| \leqslant a$. 

\item Define $\mathbb{Q}_{k}=\left\{ \mathbf{q}_{ki}\right\} $ and $\mathbb{R%
}_{k}=\mathbb{R}_{k-1}\backslash \mathbb{Q}_{k}$.
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }\mathbb{=}\left\{ 
\mathbf{q}_{1}^{\prime },...,\mathbf{q}_{k}^{\prime }\right\} $, number of
clusters $k$.

\end{mdframed}
\vspace{0.3cm}

%New points that are added to the vicinities of the cluster
%%centers at the distance smaller than $a$ do not change the basis
%(oversampling).

The construction of training subsets in the case of multiple scales requires
further modification of the algorithm.
Starting with the coarsest scale, $h_{1}$, $k_{1}$ centers can be found using the $k$-center algorithm with distance
parameter $a_{1}=\gamma h_{1}$. 
%There can be two choices then, either let
%exist basis functions with the same center and different scales, or have all
%centers different. Both choices, seems, are valid, while we prefer the
%latter case.
In our approach, we select the bases % as a subset of functions centered at
%all input points, 
such that each input point can serve as a center of only one
basis function. In this way, $k_{1}$ cluster centers of scale $h_{1}$ should
be removed from the initial training set to proceed further. Next, we
partition the remaining set using a $k$-center algorithm with distance
parameter $a_{2}=\gamma h_{2}$ and determine $k_{2}$ cluster centers. After
removal of these points we repeat the process until scale $h_{S}$ is reached
at which we determine $k_{S}$ cluster centers and stop the process. 
The algorithm is described below.

\vspace{0.3cm}
\begin{mdframed}

\center{\bf Algorithm \#2: Determination of cluster centers in multiple scales}
\vspace{0.3cm}



{\bf Input:} Set of training points $\mathbb{Q}=\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, set of scales $\mathbb{H=}\left\{ h_{1},...,h_{S}\right\} $, parameter $\gamma $. 


\begin{enumerate}
\item Define $\mathbb{R=Q};$

\item Do steps 3 to 4 for $s=1,...,S;$

\item Execute Algorithm \#1 with input $\mathbb{R}$ and max cluster radius $%
a=\gamma h_{s}$ and get cluster centers $\mathbb{Q}_{s}^{\prime }$ and
number of clusters $k_{s};$

\item Set $\mathbb{R=R}\backslash \mathbb{Q}_{s}^{\prime }.$
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }=\mathbb{\cup Q}%
_{s}^{\prime }$, $\mathbb{Q}_{s}^{\prime }=\left\{ \mathbf{q}_{1}^{(s)\prime
},...,\mathbf{q}_{k_{s}}^{(s)\prime }\right\} $, number of clusters for each
scale $k_{s}$, $s=1,...,S$.

\end{mdframed}
\vspace{0.3cm}


\begin{figure}
\centering
\pic{0.4}{figures/mgp2d1.png}~~
\pic{0.4}{figures/mgp2d2.png}
\caption{The separation of 500 random points distributed inside a unit square into clusters.
The cluster centres are shown in yellow; points belonging to different clusters are in different shades of grey. Left: small $h_n$. Right: large $h_n$.}\label{mgp2d1}
\end{figure}

Figure \ref{mgp2d1} illustrates the separated of a 2-dimensional dataset into clusters.
In principle, one can use the process even further until all the points in the training set become the cluster centers at some
scale ({\em i.e.} $D=N$).
However, as mentioned above, the reduction of the basis, or sparsification of the system matrix~\ref{which_eqn} is 
important to reduce the computational complexity of the problem.

\section{Complexity}
 The asymptotic complexity of algorithm \#1 is $O\left( Nk\right) $ and that of algorithm \#2 is $O\left( ND\right) $. 
While fast neighbor search methods~\cite{can_you_find_a_ref} can accelerate these algorithms, it has to be noted that
the overall computational cost of the regression will be dominated by the training and evaluation costs. 
It is thus instructive to discuss the complexities
of different algorithms available for training and testing. It is pertinent to examine the costs when 
$D\ll N$.  

\subsection{Training}

The goal of the training stage is to determine quantities necessary for computations on the
testing stage. In this process, two types of computations should be recognized. First,
precomputations when the set of hyperparameters is given and,
second, the optimization problem to determine the hyperparameters.

To accomplish the first task, we consider two equaivalent forms for
computation of the predictive mean and variance given by Eqs (\ref{p6}) and (%
\ref{p11}). The difference here is that expression in Eq. (\ref{p6}) are
given in terms of $D\times D$ matrices and $D\times 1$ vectors, while in Eq.
(\ref{p11}) one should operate with $N\times N$ and $N\times 1$ objects.
Respectively, the methods can be referenced as ``method $D$'' and ``method $N
$''. In both cases one should, first, form the matrix $\Phi $, and then either the $%
D\times D$ marix $\Sigma ^{-1}$, Eq. (\ref{p5}) or $N\times N$ matrix $%
K+\sigma ^{2}I$, Eq. (\ref{p10}). According to Eqs (\ref{m2}) and (\ref{m3})
the costs of this step are $O\left( ND^{2}\right) $ and $O\left(
N^{2}D\right) $, respectively. Note that these costs are much larger that $%
O\left( ND\right) $, required for determination of the basis function
centers using the $k$-center type algorithm described above. Second, weights 
$\overline{\mathbf{w}}$ from Eq. (\ref{p5}) or $\mathbf{\alpha }$ from Eq. (%
\ref{p12}) should be found. This requires solution of either $D\times D$ or $%
N\times N$ system. If solutions are performed using straightforward methods,
the costs are $O\left( D^{3}+ND\right) $ (which is the cost of solution plus
the cost of matrix-vector multiplication $\mathbf{\Phi y}$) and $O\left(
N^{3}\right) $, respectively. Note that the former cost is smaller than the
cost of formation of the system matrix $\Sigma ^{-1}$, while the latter cost
is larger than the cost of obtaining $K+\sigma ^{2}I.$ Third, the inverses $%
\Sigma $ and $\left( K+\sigma ^{2}I\right) ^{-1}$ should be found, or
efficient decomposition enabling solution of the system with multiple right
hand sides should be used. The Cholesky decomposition is usual for the
kernel matrices~\cite{rbfgp2} and it also can be used
for symmetric positively defininte matrix $\Sigma ^{-1}$,%
\begin{equation}
\Sigma ^{-1}=L_{D}L_{D}^{T},\quad K+\sigma ^{2}I=L_{N}L_{N}^{T},  \label{m6}
\end{equation}%
where $L_{D}$ and $L_{N}$ are lower triangular matrices. The decompositions
can be performed with costs $O\left( D^{3}\right) $ and $O\left(
N^{3}\right) $, respectively. Note that the Cholesky decompositions can be
used also to solve the systems for $\overline{\mathbf{w}}$ and $\mathbf{%
\alpha }$, in which case the complexity of solution becomes $O\left(
D^{2}+ND\right) $ and $O\left( N^{2}\right) $, respectively. However, this
does not change the overal cost of solution mentioned earlier, as the cost
of the Cholesky decomposition should be added to this. 

The second task requires computation of the log marginal likelihood.
Equation (\ref{p7}) is appropriate for this case for the case when matrix $%
K+\sigma ^{2}I=\Sigma _{l}$ is computed and decomposed as provided by Eq. (%
\ref{m6}). In this case we have%
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2}\mathbf{y}^{T}\mathbf{\alpha }%
-\log \left| L_{N}\right| -\frac{N}{2}\log \left( 2\pi \right) ,\quad \log
\left| L_{N}\right| =\sum_{n=1}^{N}\log L_{N,nn}  \label{m7}
\end{equation}%
The cost to compute the first term is $O(N)$ and the cost to compute the
second term is also $O(N),$ since this is a sum of logarithms of the
diagonal elements of $L_{N}$ denoted as $L_{N,nn}$. However this form is not
consistent with the idea of use $D\times D$ matrices, since the Cholesky
decomposition of $K+\sigma ^{2}I$ is too expensive compared to the other
computations. This problem can be fixed with the aid of the following lemma.

\begin{lemma}
Determinants of matrices $\Sigma $ and $\Sigma _{l}$ defined by Eqs (\ref{p5}%
) and (\ref{p6}) are related as%
\begin{equation}
\frac{1}{\sigma ^{2N}}\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }=\frac{1}{\left| \Sigma _{l}\right| }.  \label{lm1}
\end{equation}

\begin{proof}
According to definition of $\Sigma _{l}$ (\ref{p6}) we have in the right
hand side of Eq. (\ref{lm1}) 
\begin{equation}
\frac{1}{\left| \Sigma _{l}\right| }=\left| \Sigma _{l}^{-1}\right| =\frac{1%
}{\sigma ^{2N}}\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| .
\label{lm2}
\end{equation}%
Note now the Sylvester determinant theorem, which states that%
\begin{equation}
\left| I_{N}+AB\right| =\left| I_{D}+BA\right| ,  \label{lm3}
\end{equation}%
where $A$ is $N\times D$ and $B$ is $D\times N$ matrices, respectively,
while $I_{N}$ and $I_{D}$ are the $N\times N$ and $D\times D$ identity
matrices. So, we have in our case%
\begin{equation}
\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| =\left| I_{N}-%
\frac{1}{\sigma ^{2}}\Phi ^{T}\left( \Sigma \Phi \right) \right| =\left|
I_{D}-\frac{1}{\sigma ^{2}}\left( \Sigma \Phi \right) \Phi ^{T}\right|
=\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right| .  \label{lm4}
\end{equation}%
From definition (\ref{p5}) we have%
\begin{eqnarray}
I &=&\Sigma \Sigma ^{-1}=\Sigma \left( \frac{1}{\sigma ^{2}}\Phi \Phi
^{T}+\Sigma _{p}^{-1}\right) ,  \label{lm5} \\
\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right|  &=&\left| \Sigma
\Sigma _{p}^{-1}\right| =\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }.  \nonumber
\end{eqnarray}%
Combining results (\ref{lm2}), (\ref{lm4}), and (\ref{lm5}), one can see
that Eq. (\ref{lm1}) holds.
\end{proof}
\end{lemma}

Now, replacing $\Sigma _{l}^{-1}\mathbf{y}$ in the first term in the righ
hand side of Eq. (\ref{p7}) with expressions for $\Sigma _{l}^{-1}$ and $%
\overline{\mathbf{w}}$ from Eqs (\ref{p5}) and (\ref{p6}) and using Eq. (\ref%
{lm1}) in the second term, we obtain 
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\frac{1}{2}\log \left|
\Sigma ^{-1}\right| -\frac{1}{2}\log \left| \Sigma _{p}\right| -\frac{N}{2}%
\log \left( 2\pi \sigma ^{2}\right) .  \label{m8}
\end{equation}%
In case $\Sigma _{p}=\sigma _{p}^{2}I$ and Cholesky decomposition of $\Sigma
^{-1}$ we obtain%
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\sum_{j=1}^{D}\log
L_{D,jj}-\frac{N}{2}\log \left( 2\pi \sigma _{p}^{2}\sigma ^{2}\right) .
\label{m9}
\end{equation}%
Here the cost of computation of the first term in the right hand side is $%
O\left( ND\right) $ and the cost of the second term is $O\left( D\right) $ ($%
L_{D,jj}$ are the diagonal elements of $L_{D}$).

Finally, we note that multidimensional optimization is usually performed
iteratively. Assuming that the number of iterations for both methods of
computation is $N_{iter}$ we can write the costs of the training steps
marked by the respective superscripts as follows%
\begin{equation}
C_{train}^{(D)}=O\left( N_{iter}D\left( N+D^{2}\right) \right) \text{,\quad\ 
}C_{train}^{(N)}=O\left( N_{iter}N^{3}\right) \text{.}  \label{m10}
\end{equation}%
This shows thatobser%
\begin{equation}
C_{train}^{(N)}/C_{train}^{(D)}=\left\{ 
\begin{array}{c}
O\left( \left( N/D\right) ^{2}\right) \text{, }D^{2}\ll N \\ 
O\left( \left( N/D\right) ^{3}\right) \text{, }D^{2}\gtrsim N%
\end{array}%
\right. \text{,}  \label{m11}
\end{equation}%
i.e. ``method $D$'' asymptotically is much faster than ``method $N$''$.$%
Particularly, in the case of substantial oversampling $D$ does not depend on 
$N$ and at large $N$ ``method $D$'' is scaled linearly with $N$, while
``method $N$'' scaled cubically with $N$.

Finally, we can put a few remarks on optimization. If in a standard single
scale optimization of the noise level $\sigma ^{2}$ and scale $h$ for
Gaussian basis functions is sufficient, the multiscale sparse optimization
may include optimization of $\sigma ^{2}$, the number of scales $S$, $S$
parameters $h_{s}$, $s=1,...,S,$ and coefficient $\gamma $, controlling the
sparsity. The number of hyperparameters reduces to $\sigma ^{2}$, $S$, $%
\beta $, and $\alpha $ for hierarchical scaling $h_{s}=h_{1}\beta ^{s-1}$, $%
s=1,...,S$. Such situation can be appropriate, for example, for
distributions characterizing fractals, when similarity of distributions is
observed at different scales. Also the number of hyperparameters can be
reduced if some additional information is available apriory.

\subsection{Testing}

The cost of testing for methods $D$ and $N$ can be estimated from Eq. (\ref%
{p6}) and Eq. (\ref{p11}) as the costs of computing of the predicive mean
and variance. Taking into account the Cholesky decomposition (\ref{m6}),
these costs can be written as%
\begin{eqnarray}
C_{mean}^{(D)} &=&O\left( MD\right) \text{,\quad\ }C_{mean}^{(N)}=O\left(
MND\right) \text{,}  \label{m12} \\
C_{var}^{(D)} &=&O\left( MD^{2}\right) \text{,\quad\ }C_{var}^{(N)}=O\left(
MN^{2}\right) \text{,}  \nonumber
\end{eqnarray}%
where $M$ is the number of test points. Here relatively high cost $%
C_{mean}^{(N)}$ is determined by $O\left( ND\right) $ cost of computation of
vector $\mathbf{k}_{\ast }$ per evaluation point of length $N$ each
component of which should be computed as a sum of $D$ terms according to Eq.
(\ref{m3}). In contrast, cost $C_{mean}^{(D)}$ is very low, as it is
determined by the cost of the dot product of vectors of length $D$ per
evaluation point. The costs for computing of variances are much higher than
the costs of computation of the means and in both methods they are
determined by the cost of solution of triangular systems of size $D\times D$
and $N\times N$ per evaluation point. So, again, it is seen that method $D$
is much faster than method $N$.


==> mgp_newNG.tex <==
\section{Multiscale sparse GP regression}
As stated earlier, the goal of the proposed GP-based regression process is to decrease the complexity of both training and testing 
and to make the prediction more robust for datasets that have a highly irregular distribution of features.
%We start with the selection of multiple values
%of the scale parameter $h$.  
%In this case, the derivation of a compact kernel or
%covariance function in infinite-dimensional feature spaces is a
%non-trivial task because of the dependence on the apriori unknown continuous scale
%distribution (in integral (\ref{p15}) $h$ should be treated as an arbitrary
%function of $\mathbf{q}^{\prime }$ in which case a closed analytic firm is
%possible only for the cases of special assumptions. On the other hand, both
%views described above can be applied to the treatment of the problem for
%finite dimensional feature spaces.

We begin with a generalization of basis functions in Eq. (\ref{p8}),%
\begin{equation}
\phi _{j}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}_{j}^{\prime
},h_{j}\right) =\exp \left( -\frac{\left\| \mathbf{q-q}_{j}^{\prime
}\right\| ^{2}}{h_{j}^{2}}\right) ,\quad j=1,...,D,\quad \mathbf{\phi }%
=\left( \phi _{1},...,\phi _{D}\right) ^{T},  \label{m1}
\end{equation}%
where each function is characterized not only by its center $\mathbf{q}_{j}$%
, but now also by a scale $h_{j}$. The need
for such a generalization may arise from the underlying physics (e.g. particle
density estimation) or from the substantial non-uniformity of the
input data distribution, which could, for instance, demand smaller scales in denser
regions.

We note that the matrix $\Phi \Phi ^{T}$ (which is required for the
computation of covariance matrix $\Sigma $ in Eq. (\ref{p5}) and the kernel matrix $K$ in Eq. (\ref{p10}))%
is given by
\begin{eqnarray}
\left( \Phi \Phi ^{T}\right) _{ij} &=&\sum_{n=1}^{N}\phi _{i}\left( \mathbf{q%
}_{n}\right) \phi _{j}\left( \mathbf{q}_{n}\right)   \label{m2} \\
&=&\sum_{n=1}^{N}\exp \left( -\frac{\left\| \mathbf{q}_{n}-\mathbf{q}%
_{i}^{\prime }\right\| ^{2}}{h_{i}^{2}}-\frac{\left\| \mathbf{q}_{n}-\mathbf{%
q}_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad i,j=1,...,D, 
\nonumber
\end{eqnarray}%
\begin{eqnarray}
k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right)  &=&K_{mn}=\sigma
_{p}^{2}\sum_{j=1}^{D}\phi _{j}\left( \mathbf{q}_{m}\right) \phi _{j}\left( 
\mathbf{q}_{n}\right)   \label{m3} \\
&=&\sigma _{p}^{2}\sum_{j=1}^{D}\exp \left( -\frac{\left\| \mathbf{q}_{m}-%
\mathbf{q}_{j}^{\prime }\right\| ^{2}+\left\| \mathbf{q}_{n}-\mathbf{q}%
_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad m,n=1,...,N.  \nonumber
\end{eqnarray}

\subsection{Sparse representations}

While $N$ training points may be available and maximum information
can be obtained when the size of the extended feature space $D=N$, we will
search for subsets of these points leading to a lower size $D<N$. 
%The rationale for this comes from observation,
%that in interpolation problems basis functions typically can be expanded
%over the other basis functions with a sufficient accuracy (prescribed,
%determined by the noise level, or other practical reasons). This is a
%demonstration of the ill-posedness of the problem, which in the GP
%regression approach, in fact, is regularized similarly to the least square
%solution for noisy data (Tikhonov regularization [\textbf{REFERENCE}]).
The size of the extended feature space is related to the accuracy of the low-rank approximation of matrix $\Phi $ built on the entire training set ({\em i.e.}
for the case $D=N$). 

Assume for a moment that we have a single scale, $%
h_{1}=...=h_{N}=h.$ If $h$ is chosen to be smaller than
the minimum distance between the training points, the matrix $\Phi $
will have a low condition number and a low
marginal likelihood. On the other end, if $h$ is
substantially larger than the maximum distance between the training points
the problem will be ill-posed and the marginal likelihood will be also low.
The optima should lie between these extremes. If the solution is not
sensitive to the removal of a few training points, a good low-rank approximation can be sought.

The fact that the $N\times N$ matrix $\Phi $ can be well-approximated with a
matrix of rank $r<N$ means that $N-r$ rows or columns of this matrix can be
expressed as a linear combination of the other rows or columns with relatively small error $\epsilon ^{\prime }$. Assuming that $r$ locations (or centers) of the radial basis functions (or Gaussians) are given and
denoting such centers by $\mathbf{q}_{j}^{\prime }$, $j=1,...,r$, we have
\begin{equation}
\phi _{n}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}%
_{n},h_{n}\right) =\sum_{j=1}^{r}\eta _{nj}\phi _{j}\left( \mathbf{q}\right)
+\epsilon _{n}^{\prime },\quad \mathbf{q}_{j}^{/}\in \mathbb{Q}^{\prime }%
\mathbb{\subset Q}\text{,\quad }n=1,...,N,  \label{m4}
\end{equation}%
where $\eta _{nj}$ are coefficients to be determined. Hence, output (Eqn. \ref{p1}), where $f$
is expanded as Eqn. \ref{p4} with $D=N$, can be written as%
\begin{eqnarray}
y\left( \mathbf{q}\right)  &=&\sum_{n=1}^{N}w_{n}\phi _{n}\left( \mathbf{q}%
\right) +\epsilon =\sum_{j=1}^{r}w_{j}^{\prime }\phi _{j}\left( \mathbf{q}%
\right) +\epsilon +\epsilon ^{\prime }\mathbf{,}  \label{m5} \\
w_{j}^{\prime } &=&\sum_{n=1}^{N}w_{n}\eta _{nj},\quad \epsilon ^{\prime
}=\sum_{n=1}^{N}w_{n}\epsilon _{n}^{\prime }.  \nonumber
\end{eqnarray}%
This shows that if $\epsilon ^{\prime }$ is lower or comparable with noise $%
\epsilon $, then a reduced basis can be used and one can simply set the
size of the extended feature space to be the rank of the low-rank
approximation, $D=r$, and coefficients $w_{j}^{\prime }$ can be determined
by solving a $D\times D$ system instead of an $N\times N$ system.

\subsection{Representative training subsets}
\label{3_2}
Let us consider now the problem of determination of the centers of the basis
functions and scales $h_{j}$. 
%Note that even in a single-scale process, $h$ is
%not known and is determined together with other hyper-parameters by maximizing the LML (\ref{p8}).
If each data-point is assigned a different scale, then the optimization problem will become unwieldy, as
$D$ hyperparameters will have to be determined. Some compromises are made, and we instead use a set of scales $h_{1},...,h_{S}$. In the
limit of $S=1$, we have a single scale model, while at $S=D$ we prescribe a
scale to each training point. To reduce the number of scales while
providing a broad spectrum of scales, we propose the use of hierarchical
scales, e.g. $h_{s}=h_{1}\beta ^{s-1}$, $s=1,...,S$, where $h_{1}$ is of the
order of the size of the computational domain and $\beta <1$ is some
dimensionless parameter controlling the scale reduction.

While there exist several randomization-based strategies to obtain a low-rank representation
by choosing $D $ representative input points~\cite{quinonero2005}, we propose a
more regular, structured approach.  For a given scale $h$, we can specify some distance $a=\gamma h$, where $%
\gamma <1$ is chosen such that
\begin{itemize}
\item The distance from any input point to a basis point is less than $a$. Such a
construction provides an approximately  uniform coverage of the entire
training set with $d$-dimensional balls of radius $a$.

\item The number of such balls is - in some sense - optimal. Note that smaller $\gamma $ results in
smaller errors $\epsilon _{n}^{\prime }$ and $\epsilon ^{\prime }$ and
larger $r$ in Eqs. (\ref{m4}) and (\ref{m5}). If $\gamma <h/a_{\min }$, where 
$a_{\min }$ is the minimal distance between the points in the training set,
then $\epsilon^{\prime }=0$ and $r=D=N$, which corresponds to a full rank
representation.
\end{itemize}

The problem of constructing an optimal set as 
described above is computationally NP-hard. However, approximate solutions 
can be obtained with a modification of the well-known $k$-means algorithm~\cite{kmeans}.
In computational geometry problems, the $k$-means algorithm partitions a domain in $d$-dimensional space into a prescribed
number, $k$, of clusters. In the present problem, the number of clusters is
unknown, but the distance parameter $a$ is prescribed. Thus, the number of
centers depends on the input point distribution and can be determined after the
algorithm is executed. Since only the cluster centers are required for the
present problem, the following algorithm is used 
\vspace{0.3cm}

\begin{mdframed}
\center{\bf Algorithm \#1: Determination of cluster centers and k}
\vspace{0.3cm}

{\bf Input:} set of training points $\mathbb{Q=}\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, max cluster radius $a$. 


\begin{enumerate}
\item Define $\mathbb{R}_{0}=\mathbb{Q}$ and set $k=0$;

\item Do steps 3 to 6 while $\mathbb{R}_{k}\neq \emptyset ;$

\item $k=k+1;$

\item Assign $\mathbf{q}_{k}^{\prime }=\mathbf{q}_{j}\in $ $\mathbb{R}_{k-1}$
(where $\mathbf{q}_{j}$ is a random point from set $\mathbb{R}_{k-1}$)

\item Find all points $\mathbf{q}_{ki}\in \mathbb{R}_{k-1}$, such that $%
\left| \mathbf{q}_{ki}-\mathbf{q}_{k}^{\prime }\right| \leqslant a$. 

\item Define $\mathbb{Q}_{k}=\left\{ \mathbf{q}_{ki}\right\} $ and $\mathbb{R%
}_{k}=\mathbb{R}_{k-1}\backslash \mathbb{Q}_{k}$.
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }\mathbb{=}\left\{ 
\mathbf{q}_{1}^{\prime },...,\mathbf{q}_{k}^{\prime }\right\} $, number of
clusters $k$.

\end{mdframed}
\vspace{0.3cm}

%New points that are added to the vicinities of the cluster
%%centers at the distance smaller than $a$ do not change the basis
%(oversampling).

The construction of training subsets in the case of multiple scales requires
further modification of the algorithm.
Starting with the coarsest scale $h_{1}$, $k_{1}$ centers can be determined using Algorithm 1 with distance
parameter $a_{1}=\gamma h_{1}$. 
%There can be two choices then, either let
%exist basis functions with the same center and different scales, or have all
%centers different. Both choices, seems, are valid, while we prefer the
%latter case.
In our approach, we select the bases % as a subset of functions centered at
%all input points, 
such that each input point can serve as a center of only one
basis function; therefore, the $k_{1}$ cluster centers of scale $h_{1}$ should
be removed from the initial training set to proceed further. Next, we
partition the remaining set using Algorithm 1 with distance
parameter $a_{2}=\gamma h_{2}$ and determine $k_{2}$ cluster centers. After
removal of these points we repeat the process until scale $h_{S}$ is reached
at which we determine $k_{S}$ cluster centers and stop the process. 
This algorithm is described below.

\vspace{0.3cm}
\begin{mdframed}

\center{\bf Algorithm \#2: Determination of cluster centers in multiple scales}
\vspace{0.3cm}



{\bf Input:} Set of training points $\mathbb{Q}=\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, set of scales $\mathbb{H=}\left\{ h_{1},...,h_{S}\right\} $, parameter $\gamma $. 


\begin{enumerate}
\item Define $\mathbb{R=Q};$

\item Do steps 3 to 4 for $s=1,...,S;$

\item Execute Algorithm \#1 with input $\mathbb{R}$ and max cluster radius $%
a=\gamma h_{s}$ and get cluster centers $\mathbb{Q}_{s}^{\prime }$ and
number of clusters $k_{s};$

\item Set $\mathbb{R=R}\backslash \mathbb{Q}_{s}^{\prime }.$
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }=\mathbb{\cup Q}%
_{s}^{\prime }$, $\mathbb{Q}_{s}^{\prime }=\left\{ \mathbf{q}_{1}^{(s)\prime
},...,\mathbf{q}_{k_{s}}^{(s)\prime }\right\} $, number of clusters for each
scale $k_{s}$, $s=1,...,S$.

\end{mdframed}
\vspace{0.3cm}


\begin{figure}
\centering
\pic{0.4}{figures/mgp2d1.png}~~
\pic{0.4}{figures/mgp2d2.png}
\caption{The separation of 500 random points distributed inside a unit square into clusters.
The cluster centers are shown in yellow; points belonging to different clusters are in different shades of gray. Left: small $h_n$. Right: large $h_n$.}\label{mgp2d1}
\end{figure}

Figure \ref{mgp2d1} illustrates the clustering of a 2-dimensional dataset.
In principle, one can use the process even further until all the points in the training set become the cluster centers at some
scale ({\em i.e.} $D=N$).
However, as mentioned above, the reduction of 
\newpage
 the basis, $D<N$, is 
important to reduce the computational complexity of the overall problem.

\section{Complexity}
 The asymptotic complexity of algorithm \#1 is $O\left( Nk\right) $ and that of algorithm \#2 is $O\left( ND\right) $. 
While fast neighbor search methods~\cite{cheng1984} can accelerate these algorithms, 
the overall computational cost of the regression is still expected to be dominated by the training and evaluation costs. 
It is thus instructive to discuss the complexities
of different algorithms available for training and testing, especially when $D\ll N$.  

\subsection{Training}

The goal of the training stage is to determine quantities necessary for computations in the
testing stage. At this point, two types of computations should be recognized: i)
pre-computations, when the set of hyperparameters is given, and ii)
the optimization problem to determine the hyperparameters.

To accomplish the first task, we consider two equivalent forms for
computing the predictive mean and variance using Eqs. (\ref{p6}) and (%
\ref{p11}). The difference is that the expressions in Eq. (\ref{p6}) are
given in terms of $D\times D$ matrices and $D\times 1$ vectors, while Eq.
(\ref{p11}) involves $N\times N$ and $N\times 1$ arrays.
The methods can be referenced as ``method $D$'' and ``method $N
$,'' respectively, and involve three common steps: 
\begin{itemize}

\item The initial step is to form the matrix $\Phi $, and then either the $%
D\times D$ matrix $\Sigma ^{-1}$ in Eq. (\ref{p5}) or the $N\times N$ matrix $%
K+\sigma ^{2}I$ in Eq. (\ref{p10}). According to Eqs. (\ref{m2}) and (\ref{m3}),
the costs of this step are $O\left( ND^{2}\right) $ and $O\left(
N^{2}D\right) $, respectively. Note that these costs are much larger than the $%
O\left( ND\right) $ required to determine the basis function
centers using the $k$-means type algorithm described in Section \ref{3_2}. 

\item The next step involves the determination of the weights 
$\overline{\mathbf{w}}$ from Eq. (\ref{p5}) or $\mathbf{\alpha }$ from Eq. (%
\ref{p12}). This requires solving either a $D\times D$ or an $%
N\times N$ system. If solutions are obtained through direct methods,
the costs are $O\left( D^{3}+ND\right) $ (the cost of the solution plus
the cost of the matrix-vector multiplication $\mathbf{\Phi y}$) and $O\left(
N^{3}\right) $, respectively. Note that the former is computationally less intensive
than forming the system matrix $\Sigma ^{-1}$, while the latter is more expensive
 than obtaining $K+\sigma ^{2}I.$ 

\item Following this, the inverses $%
\Sigma $ and $\left( K+\sigma ^{2}I\right) ^{-1}$ should be determined\footnote{Alternatively,
efficient decompositions enabling solutions with multiple right
hand sides can be used.}. The Cholesky decomposition is typically used in this situation~\cite{rbfgp2};
\begin{equation}
\Sigma ^{-1}=L_{D}L_{D}^{T},\quad K+\sigma ^{2}I=L_{N}L_{N}^{T},  \label{m6}
\end{equation}%
where $L_{D}$ and $L_{N}$ are lower triangular matrices. The decompositions
can be performed with costs $O\left( D^{3}\right) $ and $O\left(
N^{3}\right) $, respectively. Note that the Cholesky decompositions can also be
used to solve the systems for $\overline{\mathbf{w}}$ and $\mathbf{%
\alpha }$, in which case the complexity of solution becomes $O\left(
D^{2}+ND\right) $ and $O\left( N^{2}\right) $, respectively. 

\end{itemize}

The second task requires the computation of the log marginal likelihood.
Eq. (\ref{p7}) is appropriate for the case when matrix $%
K+\sigma ^{2}I=\Sigma _{l}$ is computed and decomposed as in Eq. (%
\ref{m6}). In this case, we have%
\begin{equation}
\log p\left( \mathbf{y}|Q\right) =-\frac{1}{2}\mathbf{y}^{T}\mathbf{\alpha }%
-\log \left| L_{N}\right| -\frac{N}{2}\log \left( 2\pi \right) ,\quad \log
\left| L_{N}\right| =\sum_{n=1}^{N}\log L_{N,nn}  \label{m7}
\end{equation}%
The cost to compute the first term is $O(N)$. The cost to compute the
second term is also $O(N),$ since this is a sum of logarithms of the
diagonal elements of $L_{N}$, denoted as $L_{N,nn}$. However, this form is not
consistent with the idea of using $D\times D$ matrices, since the complexity of the Cholesky
decomposition of $K+\sigma ^{2}I$ is $O(N^3)$ and thus dominates the overall computational expense.
 This problem can be resolved with the aid of the following lemma.

\begin{lemma}
Determinants of matrices $\Sigma $ and $\Sigma _{l}$, defined by Eqs. (\ref{p5}%
) and (\ref{p6}), are related as%
\begin{equation}
\frac{1}{\sigma ^{2N}}\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }=\frac{1}{\left| \Sigma _{l}\right| }.  \label{lm1}
\end{equation}

\begin{proof}
According to the definition of $\Sigma _{l}$ (\ref{p6}), we have in the right
hand side of Eq. (\ref{lm1}) 
\begin{equation}
\frac{1}{\left| \Sigma _{l}\right| }=\left| \Sigma _{l}^{-1}\right| =\frac{1%
}{\sigma ^{2N}}\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| .
\label{lm2}
\end{equation}%
Note now the Sylvester determinant theorem, which states that%
\begin{equation}
\left| I_{N}+AB\right| =\left| I_{D}+BA\right| ,  \label{lm3}
\end{equation}%
where $A$ is an $N\times D$ matrix and $B$ is $D\times N$,
while $I_{N}$ and $I_{D}$ are the $N\times N$ and $D\times D$ identity
matrices. Thus, we have in our case%
\begin{equation}
\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| =\left| I_{N}-%
\frac{1}{\sigma ^{2}}\Phi ^{T}\left( \Sigma \Phi \right) \right| =\left|
I_{D}-\frac{1}{\sigma ^{2}}\left( \Sigma \Phi \right) \Phi ^{T}\right|
=\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right| .  \label{lm4}
\end{equation}%
From Eq. (\ref{p5}) we have%
\begin{eqnarray}
I &=&\Sigma \Sigma ^{-1}=\Sigma \left( \frac{1}{\sigma ^{2}}\Phi \Phi
^{T}+\Sigma _{p}^{-1}\right) ,  \label{lm5} \\
\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right|  &=&\left| \Sigma
\Sigma _{p}^{-1}\right| =\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }.  \nonumber
\end{eqnarray}%
Combining results (\ref{lm2}), (\ref{lm4}), and (\ref{lm5}), one can see
that Eq. (\ref{lm1}) holds.
\end{proof}
\end{lemma}

Now, replacing $\Sigma _{l}^{-1}\mathbf{y}$ in the first term in the right-hand side of Eq. (\ref{p7}) with expressions for $\Sigma _{l}^{-1}$ and $%
\overline{\mathbf{w}}$ from Eqs. (\ref{p5}) and (\ref{p6}) and using Eq. (\ref%
{lm1}) in the second term, we obtain 
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\frac{1}{2}\log \left|
\Sigma ^{-1}\right| -\frac{1}{2}\log \left| \Sigma _{p}\right| -\frac{N}{2}%
\log \left( 2\pi \sigma ^{2}\right) .  \label{m8}
\end{equation}%
In the case of $\Sigma _{p}=\sigma _{p}^{2}I$ and using the Cholesky decomposition of $\Sigma
^{-1}$, we obtain%
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\sum_{j=1}^{D}\log
L_{D,jj}-\frac{N}{2}\log \left( 2\pi \sigma _{p}^{2}\sigma ^{2}\right) .
\label{m9}
\end{equation}%
Here, the cost of computing the first term on the right hand side is $%
O\left( ND\right) $, and the cost of the second term is $O\left( D\right) $.

Multi-dimensional optimization is usually an iterative process.
 Assuming that the number of iterations for both methods of
computation is $N_{iter}$, we can write the costs of the training steps
marked by the respective superscripts as follows%
\begin{equation}
C_{train}^{(D)}=O\left( N_{iter}D\left( N+D^{2}\right) \right) \text{,\quad\ 
}C_{train}^{(N)}=O\left( N_{iter}N^{3}\right) \text{.}  \label{m10}
\end{equation}%
This shows that%
\begin{equation}
C_{train}^{(N)}/C_{train}^{(D)}=\left\{ 
\begin{array}{c}
O\left( \left( N/D\right) ^{2}\right) \text{, }D^{2}\ll N \\ 
O\left( \left( N/D\right) ^{3}\right) \text{, }D^{2}\gtrsim N%
\end{array}%
\right. \text{,}  \label{m11}
\end{equation}%
i.e. ``method $D$'' is asymptotically speaking much faster than ``method $N$.''%
Particularly, in the case of substantial oversampling, $D$ does not depend on 
$N$, and at large $N$ ``method $D$'' scales linearly with $N$ whereas
``method $N$'' scales as $N^3$.

%Finally, we can put a few remarks on optimization. If in a standard single
%scale optimization of the noise level $\sigma ^{2}$ and scale $h$ for
%Gaussian basis functions is sufficient, the multiscale sparse optimization
%may include optimization of $\sigma ^{2}$, the number of scales $S$, $S$
%parameters $h_{s}$, $s=1,...,S,$ and coefficient $\gamma $, controlling the
%sparsity. The number of hyperparameters reduces to $\sigma ^{2}$, $S$, $%
%\beta $, and $\alpha $ for hierarchical scaling $h_{s}=h_{1}\beta ^{s-1}$, $%
%s=1,...,S$. 

\subsection{Testing}

The cost of testing for methods $D$ and $N$ can be estimated from Eq. (\ref%
{p6}) and Eq. (\ref{p11}) as the costs of computing the predictive mean
and variance. Taking into account the Cholesky decomposition (\ref{m6}),
these costs can be written as%
\begin{eqnarray}
C_{mean}^{(D)} &=&O\left( MD\right) \text{,\quad\ }C_{mean}^{(N)}=O\left(
MND\right) \text{,}  \label{m12} \\
C_{var}^{(D)} &=&O\left( MD^{2}\right) \text{,\quad\ }C_{var}^{(N)}=O\left(
MN^{2}\right) \text{,}  \nonumber
\end{eqnarray}%
where $M$ is the number of test points. Here, the relatively high cost $%
C_{mean}^{(N)}$ is determined by the $O\left( ND\right) $ cost of computing the vector $\mathbf{k}_{\ast }$, a vector of length $N$ where each component is computed as a sum of $D$ terms according to Eq.
(\ref{m3}). In contrast, cost $C_{mean}^{(D)}$ is very low, as it is
determined by the cost of the dot product of vectors of length $D$ per
evaluation point. The costs for computing variances are much higher than
the costs for computing means, and in both methods they are
determined by the cost of solving triangular systems of size $D\times D$
and $N\times N$ \emph{per} evaluation point. Again, it is seen that method $D$
is much faster than method $N$.


==> mgp_revised_NG_text.tex <==

\section{Multiscale sparse GP regression}

As stated earlier, the goal of the proposed GP-based regression process is
to decrease the complexity of both training and testing and to make the
prediction more robust for datasets that have a highly irregular
distribution of features. 

We consider Gaussian basis functions,%
\begin{equation}
\phi _{j}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}_{j}^{\prime
},h_{j}\right) =\exp \left( -\frac{\left\| \mathbf{q-q}_{j}^{\prime
}\right\| ^{2}}{h_{j}^{2}}\right) ,\quad j=1,...,D,\quad \mathbf{\phi }%
=\left( \phi _{1},...,\phi _{D}\right) ^{T},  \label{m1}
\end{equation}%
where each function is characterized not only by its center $\mathbf{q}_{j}$%
, but now also by a scale $h_{j}$. The need for multiple scales may arise
from the underlying physics (e.g. particle density estimation) or from the
substantial non-uniformity of the input data distribution, which could, for
instance, demand smaller scales in denser regions. Note that the matrix $%
\Phi \Phi ^{T}$ in Eq. (\ref{p5}) and the kernel matrix $K$ in Eq. (\ref{p10}%
) are given by 
\begin{eqnarray}
\left( \Phi \Phi ^{T}\right) _{ij} &=&\sum_{n=1}^{N}\phi _{i}\left( \mathbf{q%
}_{n}\right) \phi _{j}\left( \mathbf{q}_{n}\right)   \label{m2} \\
&=&\sum_{n=1}^{N}\exp \left( -\frac{\left\| \mathbf{q}_{n}-\mathbf{q}%
_{i}^{\prime }\right\| ^{2}}{h_{i}^{2}}-\frac{\left\| \mathbf{q}_{n}-\mathbf{%
q}_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad i,j=1,...,D, 
\nonumber
\end{eqnarray}%
\begin{eqnarray}
k\left( \mathbf{q}_{m},\mathbf{q}_{n}\right)  &=&K_{mn}=\sigma
_{p}^{2}\sum_{j=1}^{D}\phi _{j}\left( \mathbf{q}_{m}\right) \phi _{j}\left( 
\mathbf{q}_{n}\right)   \label{m3} \\
&=&\sigma _{p}^{2}\sum_{j=1}^{D}\exp \left( -\frac{\left\| \mathbf{q}_{m}-%
\mathbf{q}_{j}^{\prime }\right\| ^{2}+\left\| \mathbf{q}_{n}-\mathbf{q}%
_{j}^{\prime }\right\| ^{2}}{h_{j}^{2}}\right) ,\quad m,n=1,...,N.  \nonumber
\end{eqnarray}

\subsection{Sparse representations}

While $N$ training points may be available and maximum information can be
obtained when the size of the extended feature space $D=N$, we will search
for subsets of these points leading to a lower size $D<N$. The size of the
extended feature space is related to the accuracy of the low-rank
approximation of matrix $\Phi $ built on the entire training set (i.e. for
the case $D=N$).

Assume for a moment that we have a single scale, $h_{1}=...=h_{N}=h.$ If $h$
is chosen to be smaller than the minimum distance between the training
points, the matrix $\Phi $ will have a low condition number and a low
marginal likelihood. On the other end, if $h$ is substantially larger than
the maximum distance between the training points the problem will be
ill-posed and the marginal likelihood will be also low. The optima should
lie between these extremes. If the solution is not sensitive to the removal
of a few training points, a good low-rank approximation can be sought.

The fact that the $N\times N$ matrix $\Phi $ can be well-approximated with a
matrix of rank $r<N$ means that $N-r$ rows or columns of this matrix can be
expressed as a linear combination of the other rows or columns with
relatively small error $\epsilon ^{\prime }$. Assuming that $r$ locations
(or centers) of the radial basis functions (or Gaussians) are given and
denoting such centers by $\mathbf{q}_{j}^{\prime }$, $j=1,...,r$, we have 
\begin{equation}
\phi _{n}\left( \mathbf{q}\right) =g\left( \mathbf{q},\mathbf{q}%
_{n},h_{n}\right) =\sum_{j=1}^{r}\eta _{nj}\phi _{j}\left( \mathbf{q}\right)
+\epsilon _{n}^{\prime },\quad \mathbf{q}_{j}^{/}\in \mathbb{Q}^{\prime }%
\mathbb{\subset Q}\text{,\quad }n=1,...,N,  \label{m4}
\end{equation}%
where $\eta _{nj}$ are coefficients to be determined. Hence, output (Eqn. %
\ref{p1}), where $f$ is expanded as Eqn. \ref{p4} with $D=N$, can be written
as%
\begin{eqnarray}
y\left( \mathbf{q}\right) &=&\sum_{n=1}^{N}w_{n}\phi _{n}\left( \mathbf{q}%
\right) +\epsilon =\sum_{j=1}^{r}w_{j}^{\prime }\phi _{j}\left( \mathbf{q}%
\right) +\epsilon +\epsilon ^{\prime }\mathbf{,}  \label{m5} \\
w_{j}^{\prime } &=&\sum_{n=1}^{N}w_{n}\eta _{nj},\quad \epsilon ^{\prime
}=\sum_{n=1}^{N}w_{n}\epsilon _{n}^{\prime }.  \nonumber
\end{eqnarray}%
This shows that if $\epsilon ^{\prime }$ is lower or comparable with noise $%
\epsilon $, then a reduced basis can be used and one can simply set the size
of the extended feature space to be the rank of the low-rank approximation, $%
D=r$, and coefficients $w_{j}^{\prime }$ can be determined by solving a $%
D\times D$ system instead of an $N\times N$ system.

\subsection{Representative training subsets}

\label{3_2} Let us consider now the problem of determination of the centers
of the basis functions and scales $h_{j}$. 
%Note that even in a single-scale process, $h$ is
%not known and is determined together with other hyper-parameters by maximizing the LML (\ref{p8}).
If each data-point is assigned a different scale, then the optimization
problem will become unwieldy, as $D$ hyperparameters will have to be
determined. Some compromises are made, and we instead use a set of scales $%
h_{1},...,h_{S}$. In the limit of $S=1$, we have a single scale model, while
at $S=D$ we prescribe a scale to each training point. To reduce the number
of scales while providing a broad spectrum of scales, we propose the use of
hierarchical scales, e.g. $h_{s}=h_{1}\beta ^{s-1}$, $s=1,...,S$, where $%
h_{1}$ is of the order of the size of the computational domain and $\beta <1$
is some dimensionless parameter controlling the scale reduction.

While there exist several randomization-based strategies to obtain a
low-rank representation by choosing $D $ representative input points~\cite%
{quinonero2005}, we propose a more regular, structured approach. For a given
scale $h$, we can specify some distance $a=\gamma h$, where $\gamma <1$ is
chosen such that

\begin{itemize}
\item The distance from any input point to a basis point is less than $a$.
Such a construction provides an approximately uniform coverage of the entire
training set with $d$-dimensional balls of radius $a$.

\item The number of such balls is - in some sense - optimal. Note that
smaller $\gamma $ results in smaller errors $\epsilon _{n}^{\prime }$ and $%
\epsilon ^{\prime }$ and larger $r$ in Eqs. (\ref{m4}) and (\ref{m5}). If $%
\gamma <h/a_{\min }$, where $a_{\min }$ is the minimal distance between the
points in the training set, then $\epsilon^{\prime }=0$ and $r=D=N$, which
corresponds to a full rank representation.
\end{itemize}

The problem of constructing an optimal set as described above is
computationally NP-hard. However, approximate solutions can be obtained with
a modification of the well-known $k$-means algorithm~\cite{kmeans}. In
computational geometry problems, the $k$-means algorithm partitions a domain
in $d$-dimensional space into a prescribed number, $k$, of clusters. In the
present problem, the number of clusters is unknown, but the distance
parameter $a$ is prescribed. Thus, the number of centers depends on the
input point distribution and can be determined after the algorithm is
executed. Since only the cluster centers are required for the present
problem, the following algorithm is used \vspace{0.3cm}

\begin{mdframed}
\center{\bf Algorithm \#1: Determination of cluster centers and k}
\vspace{0.3cm}

{\bf Input:} set of training points $\mathbb{Q=}\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, max cluster radius $a$. 


\begin{enumerate}
\item Define $\mathbb{R}_{0}=\mathbb{Q}$ and set $k=0$;

\item Do steps 3 to 6 while $\mathbb{R}_{k}\neq \emptyset ;$

\item $k=k+1;$

\item Assign $\mathbf{q}_{k}^{\prime }=\mathbf{q}_{j}\in $ $\mathbb{R}_{k-1}$
(where $\mathbf{q}_{j}$ is a random point from set $\mathbb{R}_{k-1}$)

\item Find all points $\mathbf{q}_{ki}\in \mathbb{R}_{k-1}$, such that $%
\left| \mathbf{q}_{ki}-\mathbf{q}_{k}^{\prime }\right| \leqslant a$. 

\item Define $\mathbb{Q}_{k}=\left\{ \mathbf{q}_{ki}\right\} $ and $\mathbb{R%
}_{k}=\mathbb{R}_{k-1}\backslash \mathbb{Q}_{k}$.
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }\mathbb{=}\left\{ 
\mathbf{q}_{1}^{\prime },...,\mathbf{q}_{k}^{\prime }\right\} $, number of
clusters $k$.

\end{mdframed}
\vspace{0.3cm}

The construction of training subsets in the case of multiple scales requires
further modification of the algorithm. Starting with the coarsest scale $%
h_{1}$, $k_{1}$ centers can be determined using Algorithm 1 with distance
parameter $a_{1}=\gamma h_{1}$. In our approach, we select the bases such
that each input point can serve as a center of only one basis function;
therefore, the $k_{1}$ cluster centers of scale $h_{1}$ should be removed
from the initial training set to proceed further. Next, we partition the
remaining set using Algorithm 1 with distance parameter $a_{2}=\gamma h_{2}$
and determine $k_{2}$ cluster centers. After removal of these points we
repeat the process until scale $h_{S}$ is reached at which we determine $%
k_{S}$ cluster centers and stop the process. This algorithm is described
below.

\vspace{0.3cm} 
\begin{mdframed}

\center{\bf Algorithm \#2: Determination of cluster centers in multiple scales}
\vspace{0.3cm}



{\bf Input:} Set of training points $\mathbb{Q}=\left\{ \mathbf{q}_{1},...,\mathbf{%
q}_{N}\right\} $, set of scales $\mathbb{H=}\left\{ h_{1},...,h_{S}\right\} $, parameter $\gamma $. 


\begin{enumerate}
\item Define $\mathbb{R=Q};$

\item Do steps 3 to 4 for $s=1,...,S;$

\item Execute Algorithm \#1 with input $\mathbb{R}$ and max cluster radius $%
a=\gamma h_{s}$ and get cluster centers $\mathbb{Q}_{s}^{\prime }$ and
number of clusters $k_{s};$

\item Set $\mathbb{R=R}\backslash \mathbb{Q}_{s}^{\prime }.$
\end{enumerate}

{\bf Output:} set of cluster centers $\mathbb{Q}^{\prime }=\mathbb{\cup Q}%
_{s}^{\prime }$, $\mathbb{Q}_{s}^{\prime }=\left\{ \mathbf{q}_{1}^{(s)\prime
},...,\mathbf{q}_{k_{s}}^{(s)\prime }\right\} $, number of clusters for each
scale $k_{s}$, $s=1,...,S$.

\end{mdframed}
\vspace{0.3cm}

\begin{figure}[tbp]
\centering \pic{0.4}{figures/mgp2d1.png}~~ \pic{0.4}{figures/mgp2d2.png}
\caption{The separation of 500 random points distributed inside a unit
square into clusters. The cluster centers are shown in yellow; points
belonging to different clusters are in different shades of gray. Left: small 
$h_n$. Right: large $h_n$.}
\label{mgp2d1}
\end{figure}

Figure \ref{mgp2d1} illustrates the clustering of a 2-dimensional dataset.
In principle, one can use the process even further until all the points in
the training set become the cluster centers at some scale (i.e. $D=N$).
However, as mentioned above, the reduction of the basis, $D<N$, is important
to reduce the computational complexity of the overall problem.

\section{Complexity}

The asymptotic complexity of algorithm \#1 is $O\left( Nk\right) $ and that
of algorithm \#2 is $O\left( ND\right) $. While fast neighbor search methods~%
\cite{cheng1984} can accelerate these algorithms, the overall computational
cost of the regression is still expected to be dominated by the training and
evaluation costs. It is thus instructive to discuss the complexities of
different algorithms available for training and testing, especially when $%
D\ll N$.

\subsection{Training}

The goal of the training stage is to determine quantities necessary for
computations in the testing stage. At this point, two types of computations
should be recognized: i) pre-computations, when the set of hyperparameters
is given, and ii) the optimization problem to determine the hyperparameters.

To accomplish the first task, we consider two equivalent forms for computing
the predictive mean and variance using Eqs. (\ref{p6}) and (\ref{p11}). The
difference is that the expressions in Eq. (\ref{p6}) are given in terms of $%
D\times D$ matrices and $D\times 1$ vectors, while Eq. (\ref{p11}) involves $%
N\times N$ and $N\times 1$ arrays. The methods can be referenced as ``method 
$D$'' and ``method $N $,'' respectively, and involve three common steps:

\begin{itemize}
\item The initial step is to form the matrix $\Phi $, and then either the $%
D\times D$ matrix $\Sigma ^{-1}$ in Eq. (\ref{p5}) or the $N\times N$ matrix 
$K+\sigma ^{2}I$ in Eq. (\ref{p10}). According to Eqs. (\ref{m2}) and (\ref%
{m3}), the costs of this step are $O\left( ND^{2}\right) $ and $O\left(
N^{2}D\right) $, respectively. Note that these costs are much larger than
the $O\left( ND\right) $ required to determine the basis function centers
using the $k$-means type algorithm described in Section \ref{3_2}.

\item The next step involves the determination of the weights $\overline{%
\mathbf{w}}$ from Eq. (\ref{p5}) or $\mathbf{\alpha }$ from Eq. (\ref{p12}).
This requires solving either a $D\times D$ or an $N\times N$ system. If
solutions are obtained through direct methods, the costs are $O\left(
D^{3}+ND\right) $ (the cost of the solution plus the cost of the
matrix-vector multiplication $\mathbf{\Phi y}$) and $O\left( N^{3}\right) $,
respectively. Note that the former is computationally less intensive than
forming the system matrix $\Sigma ^{-1}$, while the latter is more expensive
than obtaining $K+\sigma ^{2}I.$

\item Following this, the inverses $\Sigma $ and $\left( K+\sigma
^{2}I\right) ^{-1}$ should be determined\footnote{%
Alternatively, efficient decompositions enabling solutions with multiple
right hand sides can be used.}. The Cholesky decomposition is typically used
in this situation~\cite{rbfgp2}; 
\begin{equation}
\Sigma ^{-1}=L_{D}L_{D}^{T},\quad K+\sigma ^{2}I=L_{N}L_{N}^{T},  \label{m6}
\end{equation}%
where $L_{D}$ and $L_{N}$ are lower triangular matrices. The decompositions
can be performed with costs $O\left( D^{3}\right) $ and $O\left(
N^{3}\right) $, respectively. Note that the Cholesky decompositions can also
be used to solve the systems for $\overline{\mathbf{w}}$ and $\mathbf{\alpha 
}$, in which case the complexity of solution becomes $O\left(
D^{2}+ND\right) $ and $O\left( N^{2}\right) $, respectively.
\end{itemize}

The second task requires the computation of the log marginal likelihood. Eq.
(\ref{p7}) is appropriate for the case when matrix $K+\sigma ^{2}I=\Sigma
_{l}$ is computed and decomposed as in Eq. (\ref{m6}). In this case, we have%
\begin{equation}
\log p\left( \mathbf{y}|Q\right) =-\frac{1}{2}\mathbf{y}^{T}\mathbf{\alpha }%
-\log \left| L_{N}\right| -\frac{N}{2}\log \left( 2\pi \right) ,\quad \log
\left| L_{N}\right| =\sum_{n=1}^{N}\log L_{N,nn}  \label{m7}
\end{equation}%
The cost to compute the first term is $O(N)$. The cost to compute the second
term is also $O(N),$ since this is a sum of logarithms of the diagonal
elements of $L_{N}$, denoted as $L_{N,nn}$. However, this form is not
consistent with the idea of using $D\times D$ matrices, since the complexity
of the Cholesky decomposition of $K+\sigma ^{2}I$ is $O(N^3)$ and thus
dominates the overall computational expense.  This problem can be resolved
with the aid of the following lemma.

\begin{lemma}
Determinants of matrices $\Sigma $ and $\Sigma _{l}$, defined by Eqs. (\ref%
{p5}) and (\ref{p6}), are related as%
\begin{equation}
\frac{1}{\sigma ^{2N}}\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }=\frac{1}{\left| \Sigma _{l}\right| }.  \label{lm1}
\end{equation}

\begin{proof}
According to the definition of $\Sigma _{l}$ (\ref{p6}), we have in the
right hand side of Eq. (\ref{lm1}) 
\begin{equation}
\frac{1}{\left| \Sigma _{l}\right| }=\left| \Sigma _{l}^{-1}\right| =\frac{1%
}{\sigma ^{2N}}\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| .
\label{lm2}
\end{equation}%
Note now the Sylvester determinant theorem, which states that%
\begin{equation}
\left| I_{N}+AB\right| =\left| I_{D}+BA\right| ,  \label{lm3}
\end{equation}%
where $A$ is an $N\times D$ matrix and $B$ is $D\times N$, while $I_{N}$ and 
$I_{D}$ are the $N\times N$ and $D\times D$ identity matrices. Thus, we have
in our case%
\begin{equation}
\left| I-\frac{1}{\sigma ^{2}}\Phi ^{T}\Sigma \Phi \right| =\left| I_{N}-%
\frac{1}{\sigma ^{2}}\Phi ^{T}\left( \Sigma \Phi \right) \right| =\left|
I_{D}-\frac{1}{\sigma ^{2}}\left( \Sigma \Phi \right) \Phi ^{T}\right|
=\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right| .  \label{lm4}
\end{equation}%
From Eq. (\ref{p5}) we have%
\begin{eqnarray}
I &=&\Sigma \Sigma ^{-1}=\Sigma \left( \frac{1}{\sigma ^{2}}\Phi \Phi
^{T}+\Sigma _{p}^{-1}\right) ,  \label{lm5} \\
\left| I-\frac{1}{\sigma ^{2}}\Sigma \Phi \Phi ^{T}\right| &=&\left| \Sigma
\Sigma _{p}^{-1}\right| =\frac{\left| \Sigma \right| }{\left| \Sigma
_{p}\right| }.  \nonumber
\end{eqnarray}%
Combining results (\ref{lm2}), (\ref{lm4}), and (\ref{lm5}), one can see
that Eq. (\ref{lm1}) holds.
\end{proof}
\end{lemma}

Now, replacing $\Sigma _{l}^{-1}\mathbf{y}$ in the first term in the
right-hand side of Eq. (\ref{p7}) with expressions for $\Sigma _{l}^{-1}$
and $\overline{\mathbf{w}}$ from Eqs. (\ref{p5}) and (\ref{p6}) and using
Eq. (\ref{lm1}) in the second term, we obtain 
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\frac{1}{2}\log \left|
\Sigma ^{-1}\right| -\frac{1}{2}\log \left| \Sigma _{p}\right| -\frac{N}{2}%
\log \left( 2\pi \sigma ^{2}\right) .  \label{m8}
\end{equation}%
In the case of $\Sigma _{p}=\sigma _{p}^{2}I$ and using the Cholesky
decomposition of $\Sigma ^{-1}$, we obtain%
\begin{equation}
\log p\left( \mathbf{y}|X\right) =-\frac{1}{2\sigma ^{2}}\left( \mathbf{y}%
-\Phi ^{T}\overline{\mathbf{w}}\right) ^{T}\mathbf{y}-\sum_{j=1}^{D}\log
L_{D,jj}-\frac{N}{2}\log \left( 2\pi \sigma _{p}^{2}\sigma ^{2}\right) .
\label{m9}
\end{equation}%
Here, the cost of computing the first term on the right hand side is $%
O\left( ND\right) $, and the cost of the second term is $O\left( D\right) $.

Multi-dimensional optimization is usually an iterative process.  Assuming
that the number of iterations for both methods of computation is $N_{iter}$,
we can write the costs of the training steps marked by the respective
superscripts as follows%
\begin{equation}
C_{train}^{(D)}=O\left( N_{iter}D\left( N+D^{2}\right) \right) \text{,\quad\ 
}C_{train}^{(N)}=O\left( N_{iter}N^{3}\right) \text{.}  \label{m10}
\end{equation}%
This shows that%
\begin{equation}
C_{train}^{(N)}/C_{train}^{(D)}=\left\{ 
\begin{array}{c}
O\left( \left( N/D\right) ^{2}\right) \text{, }D^{2}\ll N \\ 
O\left( \left( N/D\right) ^{3}\right) \text{, }D^{2}\gtrsim N%
\end{array}%
\right. \text{,}  \label{m11}
\end{equation}%
i.e. ``method $D$'' is asymptotically speaking much faster than ``method $N$%
.''Particularly, in the case of substantial oversampling, $D$ does not
depend on $N$, and at large $N$ ``method $D$'' scales linearly with $N$
whereas ``method $N$'' scales as $N^3$.

%Finally, we can put a few remarks on optimization. If in a standard single
%scale optimization of the noise level $\sigma ^{2}$ and scale $h$ for
%Gaussian basis functions is sufficient, the multiscale sparse optimization
%may include optimization of $\sigma ^{2}$, the number of scales $S$, $S$
%parameters $h_{s}$, $s=1,...,S,$ and coefficient $\gamma $, controlling the
%sparsity. The number of hyperparameters reduces to $\sigma ^{2}$, $S$, $%
%\beta $, and $\alpha $ for hierarchical scaling $h_{s}=h_{1}\beta ^{s-1}$, $%
%s=1,...,S$. 

\subsection{Testing}

The cost of testing for methods $D$ and $N$ can be estimated from Eq. (\ref%
{p6}) and Eq. (\ref{p11}) as the costs of computing the predictive mean and
variance. Taking into account the Cholesky decomposition (\ref{m6}), these
costs can be written as%
\begin{eqnarray}
C_{mean}^{(D)} &=&O\left( MD\right) \text{,\quad\ }C_{mean}^{(N)}=O\left(
MND\right) \text{,}  \label{m12} \\
C_{var}^{(D)} &=&O\left( MD^{2}\right) \text{,\quad\ }C_{var}^{(N)}=O\left(
MN^{2}\right) \text{,}  \nonumber
\end{eqnarray}%
where $M$ is the number of test points. Here, the relatively high cost $%
C_{mean}^{(N)}$ is determined by the $O\left( ND\right) $ cost of computing
the vector $\mathbf{k}_{\ast }$, a vector of length $N$ where each component
is computed as a sum of $D$ terms according to Eq. (\ref{m3}). In contrast,
cost $C_{mean}^{(D)}$ is very low, as it is determined by the cost of the
dot product of vectors of length $D$ per evaluation point. The costs for
computing variances are much higher than the costs for computing means, and
in both methods they are determined by the cost of solving triangular
systems of size $D\times D$ and $N\times N$ \emph{per} evaluation point.
Again, it is seen that method $D$ is much faster than method $N$.

==> results_Orig.tex <==
\section{Numerical Results}
\subsection{1-D Sine Function}
The simplest numerical example on which ML was tested was a noisy sine function, $y = \sin(8\pi q) + \mc{N}(0,0.1)$, with $q$ limited to $[0,1]$. Two cases are tested: the first with training values for $q$ chosen from a uniform distribution, and the second with $q$ chosen randomly from normal distributions centred around $0.1$, $0.5$, and $0.9$. 300 training points are used in each case. Prior to usage in GP, training inputs and outputs are scaled to $[0,1]$. Test inputs are scaled using the range and minimum of $\mb{Q}_{\mr{train}}$, and the results from learning are scaled back using the range and minimum of $\mb{Y}_{\mr{train}}$.

In addition to Figure \ref{mgp2d1} in the previous section, Figures \ref{sinerand} and \ref{sinerandn} further illustrate the process of selecting cluster centres. They are for the uniform and clustered input cases, respectively. In each figure, the leftmost plot shows the cluster centres chosen with $h_k=h_1$, the middle plot centres with $h_2$, and the rightmost centres with $h_3$. Since $h_k$ decreases with $k$, more centres are chosen with increasing $k$ because they are not constrained to be as far apart from each other. The centres are randomly chosen, so they are not evenly distributed across the domain, but the spacing between them is fairly regular. With these sample parameters, approximately 50 centres cumulative are selected across these three scales, and the rest of the training points are disregarded. This means the size of the training dataset has effectively been reduced from 300 to 50. The consequent increase in speed is very important when coupling a ML model to a turbulence model, since numerous test points must be evaluated per iteration of the flow solver.

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerand.pdf}
		\caption{Clustering produced by MGP for uniform distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points, signifying points that were within $h_k$ of the cluster centre at the time of its selection. $h_0=4$, $r = 2$. } \label{sinerand}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerandn.pdf}
		\caption{Clustering produced by MGP for clustered distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points within $h_k$ of the centre. $h_0=4$, $r = 2$ as before. }  \label{sinerandn}
\end{figure}

Following this graphical example, the optimal hyperparameters for each method are found through minimising the LML, and the results of testing on new sets of randomly selected $q_{\mr{test}}$ using the optimised ML methods are summarised in Table \ref{sineerr}. No validation sets were used, meaning that all the original training points were considered when computing the LML. For the clustered case, MGP used only 20 cluster centres out of 300 original training points to achieve this result, plotted in Figures \ref{sineures} and \ref{sinecres}. Despite the more than tenfold reduction in the number of cluster centres vesus the number of training points, the speedup is not precisely linear due to computational overhead. Figures \ref{sineuline} and \ref{sinecline} depict the ML output $f(q_{\mr{test}})$ versus the original $y_{\mr{test}}$. In general, the variance of the output appears larger near the extrema of the sine function and smaller near zero, the same behaviour as observed in Figures \ref{sineures} and \ref{sinecres}.

\begin{table}
\caption{Normalised test errors for ML methods, defined as $||\mb{Y}_{\mr{test}} - f(\mb{Q}_{\mr{test}})||/||\mb{Y}_{\mr{test}}||$. 1000 uniformly spaced test points on $[0,1]$ were used.  Time is test time in seconds. Training time is part of preprocessing and thus less relevant.}
\label{sineerr}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Uniform input & 0.0257 & $7.7\times10^{-3}$ & 0.0407 & $2.4\times10^{-3}$ \\ \hline
    Clustered input & 0.0516 & $9.6\times10^{-3}$ & 0.0716 & $1.7\times10^{-3}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sineuniform.pdf}
		\caption{Uniform distribution testing results for all methods. Black line is the original function, black dots are training points with noise added. Blue line is the ML output. For GP and MGP, shaded red regions indicate confidence intervals of $\pm1\sigma$. }  \label{sineures}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinecluster.pdf}
		\caption{Clustered distribution testing results for all methods. Black line is the original function, black dots are training points. Blue line is the ML output. For GP and MGP, red regions are confidence intervals of $\pm1\sigma$. There are noticeable divergences from the true function, especially near maxima and minima, compared to the uniformly distributed training point case.}  \label{sinecres}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandline.pdf}
		\caption{Test output $y_{\mr{test}}$ versus ML output $f(q_{\mr{test}})$ for uniformly distributed test points. The red line is $f(q_{\mr{test}}) = y_{\mr{test}}$. Shaded red region is $\pm 0.1$ from the red line, i.e. one standard deviation for the noise in the training data.}  \label{sineuline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandnline.pdf}
		\caption{$y_{\mr{test}}$ versus $f(q_{\mr{test}})$ for clustered test points. Red line is $f(q_{\mr{test}}) = y_{\mr{test}}$, shaded red region is $\pm 0.1$ from the red line. Ordinary GP is clearly deviating from the line, likely in locations lacking training points.}  \label{sinecline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08.pdf}
		\caption{Tradeoffs in speed and accuracy for performing MGP on uniformly distributed data. Blue points are for randomly-selected hyperparameters, and orange `x's are for using the optimal hyperparameters from maximising the LML. The two plotted have $K=5$ and $K=6$, with the former having less error. The black `x' is a sample GP for comparison. The error for MGP rises very sharply as test time decreases beyond a certain point.}  \label{sineupareto}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08randn.pdf}
		\caption{Tradeoffs in speed and accuracy for MGP on clustered data. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=5$ and $K=6$, the former having lower error. Black is a sample GP result for comparison.}  \label{sinecpareto}
\end{figure}

On a final note, Figures \ref{sineupareto} and \ref{sinecpareto} show that optimal parameters selected through maximising the LML are also near optimal according to the test error, validating the use of LML for hyperparameter optimisation. Comparing this to the numerical results in Table \ref{sineerr}, the tradeoff between speed and accuracy is shown to be worthwhile for the majority of cases, since the percentage decrease in test time is greater than the increase in error. Of note is the fact that as number of scales $K$ increases, the test error increases sharply for the clustered training data, but does not increase much for the evenly distributed training data. In addition, for values of $K$ smaller than $5$, the test error also increases quickly to the point where the optimal results for $K\leq4$ are not visible in the figures. This suggests that it is both somewhat easy to overfit using MGP, and also to select too few training points. 

\subsection{2-D Curved Channel}
In this section, further numerical results for turbulent flow through 2-D convex and concave channels are provided. The freestream Reynolds number is about 0.6 million. The channel has a turn angle of 90 degrees, and the radius of curvature is unity. 

The Spalart-Allmaras model is applied here. The baseline SA model solves for turbulent viscosity $\hat{\mu}_t$ through the following equation:
\begin{equation}
\frac{\mathrm{D}\hat{\nu}}{\mathrm{D}t} = P_{\nu} - D_{\nu} + \frac{1}{\sigma}\left[\nabla\cdot\left(\left(\frac{\hat{\mu}}{\overline{\rho}} + \hat{\nu}\right)\nabla\hat{\nu}\right) + c_{b2}(\nabla\hat{\nu})^2\right]
\label{saeqnorig}
\end{equation}
where
\begin{equation}
\hat{\mu}_t = \overline{\rho}\hat{\nu}f_{\nu1}
\end{equation}
$P_{\nu}$ and $D_{\nu}$ are the production and destruction terms.
An altered version of the baseline SA model, conventionally named SA-RC\cite{sarc}, was devised in order to better account for rotation and curvature effects. SA-RC only differs from the original SA model by the presence of the extra multiplicative factor $f_{r1}$ in its production term. The production and destruction terms for SA-RC defined as:
\begin{equation}
P_{\nu} = c_{b1}f_{r1}\hat{\Omega}\hat{\nu} \qquad \qquad%
D_{\nu} = c_{w1}f_w \left(\frac{\hat{\nu}}{d}\right)^2
\end{equation}
with 
\begin{equation}
f_{r1} = (1+c_{r1})\left(\frac{2r^*}{1+r^*}\right)[1-c_{r3}\tan^{-1}(c_{r2}\hat{r})]-c_{r1}
\end{equation}
The functions $f_{\nu1}$, $\hat{\Omega}$, $r^*$ $\hat{r}$, and $f_w$ are analytical. $d$ is the distance from the current point to the nearest solid boundary. $c_{b1}$, $c_{b2}$, $c_{w1}$, $\sigma$, $c_{r1}$, $c_{r2}$, and $c_{r3}$ are constants.

For the data-driven approach to turbulence modelling presented in this work, a field variable $\alpha$ is introduced. $\alpha$ modifies the original SA-RC model in Eq. (\ref{saeqnorig}) as follows:
\begin{equation}
\frac{\mathrm{D}\hat{\nu}}{\mathrm{D}t} = \alpha + P_{\nu} - D_{\nu} + \frac{1}{\sigma}\left[\nabla\cdot\left(\left(\frac{\hat{\mu}}{\overline{\rho}} + \hat{\nu}\right)\nabla\hat{\nu}\right) + c_{b2}(\nabla\hat{\nu})^2\right]
\end{equation}

$\alpha$ can take the form of $\alpha_{\mr{SARC}}$ or $\alpha_{\mr{LES}}$. $\alpha_{\mr{SARC}}$ refers to the difference in production terms between SA and SA-RC, and $\alpha_{\mr{LES}}$ refers to the difference between SA and the production term that is needed for the output of RANS to match LES in terms of $C_f$. $\alpha_{\mr{SARC}}$ is an analytical function of $\hat{r}$, $r^*$, $\hat{\Omega}$, and $\hat{\nu}$, whereas $\alpha_{\mr{LES}}$ is more complicated. Therefore, it is necessary to use parameters in addition to the four aforementioned for $\alpha_{\mr{LES}}$. In this work, the additional parameter was chosen to be $d$, the distance from the point to the nearest wall. For consistency, $d$ was also used in the training of $\alpha_{\mr{SARC}}$. 

Even with additional parameters, the 2-D channel is more difficult to learn than the previous examples. To simplify the problem, training points were reduced to those for which $\alpha$ was nonzero, essentially limiting training points to those within the boundary layer. Finally, since the number of grid points is still large even with this restriction, 5 percent, or approximately 2000, of the total number of points were used for training in each case. 

First, it is prudent to verify that the function $f_{r1}$ can be learned with $\hat{r}$ and $r^*$ as the inputs. Only if this is learnable can one expect $\alpha$ to be learnable as well. Fortunately, the function is smooth and continuous for the involved range of inputs. Similar to the analytical example in the previous section, inputs and training outputs are scaled to $[0,1]$ for learning purposes. The results are plotted in Figures 
\ref{ccf1} and \ref{cvf1}, and numerical results are in Table \ref{channelf1err}. 

\begin{figure}
\centering
\pic{0.6}{figures/ccf1line.pdf}
\caption{Test results for $f_{r1}$ in the concave channel. The red line is the exact result.}\label{ccf1}
\end{figure}

\begin{figure}
\centering
\pic{0.6}{figures/cvf1line.pdf}
\caption{Test results for $f_{r1}$ in the convex channel. There is more deviation from the correct output compared to the concave channel. }\label{cvf1}
\end{figure}

\begin{table}
\caption{Numerical results for learning $f_{r1}$. Approximately $300$ randomly selected test points from each geometry were used.  Error is as previously defined in Table \ref{sineerr}. Time is test time in seconds.}
\label{channelf1err}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Concave channel & 0.0017 & $1.7\times10^{-2}$ & 0.0019 & $4.0\times10^{-3}$ \\ \hline
    Convex channel & 0.0044 & $1.9\times10^{-2}$ & 0.0163 & $3.2\times10^{-3}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/ccf1pareto.pdf}
		\caption{Tradeoffs in ML performance for $f_{r1}$ in a concave channel. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=[7,8,9]$, and black is the optimal GP result for comparison. }  \label{ccf1pareto}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/cvf1pareto.pdf}
	\caption{Tradeoffs in ML performance for $f_{r1}$ in a convex channel. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=[7,8]$, and black is the optimal GP result [redo this if time, could show upward trend in bottom branch of pareto like in concave case]. }   \label{cvf1pareto}
\end{figure}

\begin{figure}
\centering
\pic{0.6}{figures/ccda.pdf}
\caption{Test results for $\alpha$ in the concave channel. Around $300$ random points were used. Red line represents the exact $\alpha$. }\label{concave}
\end{figure}

\begin{figure}
\centering
\pic{0.6}{figures/cvda.pdf}
\caption{Test results for $\alpha$ in the convex channel. As with $f_{r1}$, the ML output is noticeably worse for MGP, though the overall error has increased for both GP and MGP.}\label{convex}
\end{figure}

\begin{table}
\caption{Test results for learning $\alpha$. Approximately $300$ randomly selected test points from each geometry were used.  Time is test time in seconds.}
\label{channelerr}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Concave channel & 0.0352 & $2.8\times10^{-2}$ & 0.0564 & $1.4\times10^{-3}$ \\ \hline
    Convex channel & 0.0789 & $2.4\times10^{-2}$ & 0.1041 & $1.7\times10^{-2}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.49}{figures/ccpareto.pdf}
	\pic{0.49}{figures/cvpareto.pdf}
		\caption{Concave and convex channel pareto plot. No matter what hyperparameters I throw at them, GP seems to be below the curve. [Temporary observation, not going into final paper unless it helps me figure out why channel error is so high]}  \label{cvpareto}
\end{figure}

\textcolor{red}{
Results section
\begin{itemize}
\item Analytical part is most complete
\item Is it helpful to compute average error and speedup from different random sets of training points, or is the scatterplot sufficient?
\end{itemize}
}

==> results_orig2.tex <==
\section{Numerical Results}
\subsection{1-D Sine Function}
The simplest numerical example on which ML was tested was a noisy sine function, $y = \sin(8\pi q) + \mc{N}(0,0.1)$, with $q$ limited to $[0,1]$. Two cases are tested: the first with training values for $q$ chosen from a uniform distribution, and the second with $q$ chosen randomly from normal distributions centred around $0.1$, $0.5$, and $0.9$. 300 training points are used in each case. Prior to usage in GP, training inputs and outputs are scaled to $[0,1]$. Test inputs are scaled using the range and minimum of $\mb{Q}_{\mr{train}}$, and the results from learning are scaled back using the range and minimum of $\mb{Y}_{\mr{train}}$.

In addition to Figure \ref{mgp2d1} in the previous section, Figures \ref{sinerand} and \ref{sinerandn} further illustrate the process of selecting cluster centres. They are for the uniform and clustered input cases, respectively. In each figure, the leftmost plot shows the cluster centres chosen with $h_k=h_1$, the middle plot centres with $h_2$, and the rightmost centres with $h_3$. Since $h_k$ decreases with $k$, more centres are chosen with increasing $k$ because they are not constrained to be as far apart from each other. The centres are randomly chosen, so they are not evenly distributed across the domain, but the spacing between them is fairly regular. With these sample parameters, approximately 50 centres cumulative are selected across these three scales, and the rest of the training points are disregarded. This means the size of the training dataset has effectively been reduced from 300 to 50. The consequent increase in speed is very important when coupling a ML model to a turbulence model, since numerous test points must be evaluated per iteration of the flow solver.

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerand.pdf}
		\caption{Clustering produced by MGP for uniform distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points, signifying points that were within $h_k$ of the cluster centre at the time of its selection. $h_0=4$, $r = 2$. } \label{sinerand}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/sine/sinerandn.pdf}
		\caption{Clustering produced by MGP for clustered distribution of inputs. Left to right: scale $k=1$, $k=2$, and $k=3$. Black crosses are cluster centres selected at each scale. Surrounding each cluster centre is a colour-coded group of training points within $h_k$ of the centre. $h_0=4$, $r = 2$ as before. }  \label{sinerandn}
\end{figure}

Following this graphical example, the optimal hyperparameters for each method are found through minimising the LML, and the results of testing on new sets of randomly selected $q_{\mr{test}}$ using the optimised ML methods are summarised in Table \ref{sineerr}. No validation sets were used, meaning that all the original training points were considered when computing the LML. For the clustered case, MGP used only 20 cluster centres out of 300 original training points to achieve this result, plotted in Figures \ref{sineures} and \ref{sinecres}. Despite the more than tenfold reduction in the number of cluster centres vesus the number of training points, the speedup is not precisely linear due to computational overhead. Figures \ref{sineuline} and \ref{sinecline} depict the ML output $f(q_{\mr{test}})$ versus the original $y_{\mr{test}}$. In general, the variance of the output appears larger near the extrema of the sine function and smaller near zero, the same behaviour as observed in Figures \ref{sineures} and \ref{sinecres}.

\begin{table}
\caption{Normalised test errors for ML methods, defined as $||\mb{Y}_{\mr{test}} - f(\mb{Q}_{\mr{test}})||/||\mb{Y}_{\mr{test}}||$. 1000 uniformly spaced test points on $[0,1]$ were used.  Time is test time in seconds. Training time is part of preprocessing and thus less relevant.}
\label{sineerr}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Uniform input & 0.0257 & $7.7\times10^{-3}$ & 0.0407 & $2.4\times10^{-3}$ \\ \hline
    Clustered input & 0.0516 & $9.6\times10^{-3}$ & 0.0716 & $1.7\times10^{-3}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sineuniform.pdf}
		\caption{Uniform distribution testing results for all methods. Black line is the original function, black dots are training points with noise added. Blue line is the ML output. For GP and MGP, shaded red regions indicate confidence intervals of $\pm1\sigma$. }  \label{sineures}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinecluster.pdf}
		\caption{Clustered distribution testing results for all methods. Black line is the original function, black dots are training points. Blue line is the ML output. For GP and MGP, red regions are confidence intervals of $\pm1\sigma$. There are noticeable divergences from the true function, especially near maxima and minima, compared to the uniformly distributed training point case.}  \label{sinecres}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandline.pdf}
		\caption{Test output $y_{\mr{test}}$ versus ML output $f(q_{\mr{test}})$ for uniformly distributed test points. The red line is $f(q_{\mr{test}}) = y_{\mr{test}}$. Shaded red region is $\pm 0.1$ from the red line, i.e. one standard deviation for the noise in the training data.}  \label{sineuline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/sine/sinerandnline.pdf}
		\caption{$y_{\mr{test}}$ versus $f(q_{\mr{test}})$ for clustered test points. Red line is $f(q_{\mr{test}}) = y_{\mr{test}}$, shaded red region is $\pm 0.1$ from the red line. Ordinary GP is clearly deviating from the line, likely in locations lacking training points.}  \label{sinecline}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08.pdf}
		\caption{Tradeoffs in speed and accuracy for performing MGP on uniformly distributed data. Blue points are for randomly-selected hyperparameters, and orange `x's are for using the optimal hyperparameters from maximising the LML. The two plotted have $K=5$ and $K=6$, with the former having less error. The black `x' is a sample GP for comparison. The error for MGP rises very sharply as test time decreases beyond a certain point.}  \label{sineupareto}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/sine/sinepareto08randn.pdf}
		\caption{Tradeoffs in speed and accuracy for MGP on clustered data. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=5$ and $K=6$, the former having lower error. Black is a sample GP result for comparison.}  \label{sinecpareto}
\end{figure}

On a final note, Figures \ref{sineupareto} and \ref{sinecpareto} show that optimal parameters selected through maximising the LML are also near optimal according to the test error, validating the use of LML for hyperparameter optimisation. Comparing this to the numerical results in Table \ref{sineerr}, the tradeoff between speed and accuracy is shown to be worthwhile for the majority of cases, since the percentage decrease in test time is greater than the increase in error. Of note is the fact that as number of scales $K$ increases, the test error increases sharply for the clustered training data, but does not increase much for the evenly distributed training data. In addition, for values of $K$ smaller than $5$, the test error also increases quickly to the point where the optimal results for $K\leq4$ are not visible in the figures. This suggests that it is both somewhat easy to overfit using MGP, and also to select too few training points. 

\subsection{2-D Curved Channel}

\begin{equation}
f_{r1} = (1+c_{r1})\left(\frac{2r^*}{1+r^*}\right)[1-c_{r3}\tan^{-1}(c_{r2}\hat{r})]-c_{r1}
\end{equation}
First, it is prudent to verify that the function $f_{r1}$ can be learned with $\hat{r}$ and $r^*$ as the inputs. 
Similar to the analytical example in the previous section, inputs and training outputs are scaled to $[0,1]$ for learning purposes. 
The results are plotted in Figures 
\ref{ccf1} and \ref{cvf1}, and numerical results are in Table \ref{channelf1err}. 

\begin{figure}
\centering
\pic{0.6}{figures/ccf1line.pdf}
\caption{Test results for $f_{r1}$ in the concave channel. The red line is the exact result.}\label{ccf1}
\end{figure}

\begin{figure}
\centering
\pic{0.6}{figures/cvf1line.pdf}
\caption{Test results for $f_{r1}$ in the convex channel. There is more deviation from the correct output compared to the concave channel. }\label{cvf1}
\end{figure}

\begin{table}
\caption{Numerical results for learning $f_{r1}$. Approximately $300$ randomly selected test points from each geometry were used.  Error is as previously defined in Table \ref{sineerr}. Time is test time in seconds.}
\label{channelf1err}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    Concave channel & 0.0017 & $1.7\times10^{-2}$ & 0.0019 & $4.0\times10^{-3}$ \\ \hline
    Convex channel & 0.0044 & $1.9\times10^{-2}$ & 0.0163 & $3.2\times10^{-3}$\\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/ccf1pareto.pdf}
		\caption{Tradeoffs in ML performance for $f_{r1}$ in a concave channel. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=[7,8,9]$, and black is the optimal GP result for comparison. }  \label{ccf1pareto}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.5}{figures/cvf1pareto.pdf}
	\caption{Tradeoffs in ML performance for $f_{r1}$ in a convex channel. Blue points are for random hyperparameters, orange are for optimal hyperparameters with $K=[7,8]$, and black is the optimal GP result [redo this if time, could show upward trend in bottom branch of pareto like in concave case]. }   \label{cvf1pareto}
\end{figure}

\textcolor{red}{
Results section
\begin{itemize}
\item Is it helpful to compute average error and speedup from different random sets of training points, or is the scatterplot sufficient?
\end{itemize}
}

\subsection{3-D Turbulent Combustion}
Turbulent combustion involves an enormous disparity in time and length scales, meaning that direct numerical simulations (DNS) are not possible
for practical problems. Large eddy simulations (LES), in which the effect of scales smaller than the mesh resolution are modeled, is often a more pragmatic
choice. A key difficulty in LES is the modeling of the subgrid scale fluxes in the species transport equations~\cite{kant1,kant2}. These terms
arise as a result of the low-pass filtering (represented by the operator $(\bar{\cdot})$) of the governing equations, and are of the form 
\[f_k = \overline{\rho u_k C}-\frac{\overline{rho u_k}\overline{\rho C}}{\bar{rho}}\]
where $\rho, u,C$ represent density, velocity and species mass fraction, respectively. 
Subgrid scale closures based on concepts from non-reacting flows, such as the equation below,\footnote{$C_s, Sc$ are typically constants, and $S_{ij} = \frac{1}{2}\left[ 
\frac{\partial u_i}{\partial x_j} + \frac{\partial u_j}{\partial x_i} \right]$ is the strain-rate tensor.}
\[f_{i} = -\frac{\overline{\rho} C_s^2 \Delta^2 \sqrt{2 \tilde{S}_{ij} \tilde{S}_{ij}}}{Sc}\frac{\partial \tilde{c}}{\partial x_k}\]
are found to be inadequate for turbulent combustion. Modeling of the scalar fluxes thus continues to be an active area of research, and many analytical models are being evaluated by the community. Reference ~\cite{chakraborthy} provides a concise summary.

%\[f_{i} = \frac{\overline{\rho}\Delta^2}{12}\frac{\partial \tilde{u}_i}{\partial x_k}\frac{\partial \tilde{c}}{\partial x_k}\]

In this example, we intend to apply machine learning to identify the model relationship. The data comes from Ref.~\cite{raman}, in which
DNS of a propagating turbulent flame is performed. The geometry is such that the premixed hydrogen-air flame propagates in the 
x-direction and forms a thin front between the burnt and unburnt gas. 


Specifically, we attempt to learn the normalised flux in the x-direction, $F_1$, as a function of seven variables:
\[F_1 = \frac{f_1}{\overline{\rho} \Delta^2} = f(\nabla \tilde{u},\nabla \tilde{c},\tilde{S})\]

A total of 1 million training points were available from the data.
Some care was taken when choosing training points. Since the flame is thin relative to the size of the domain, the majority of points lie outside the region where $F_1$ is nonzero. To mitigate this disadvantageous distribution, 80 percent of the training points were randomly chosen from the data with $f_1 > 0.05$, and 20 percent were chosen from data with $f_1 \leq 0.05$, i.e. outside the flame. About 2500 training points were used in total. For testing, a single $x-y$ plane of around 6500 points was set aside.

\begin{table}
\caption{Numerical results for learning $F_1$ in the flame. Error is as previously defined in Table \ref{sineerr}. Time is test time in seconds.}
\label{comberr}
\centering
  \begin{tabular}{| l | c | c | c | c |}
    \hline
    & \multicolumn{2}{c|}{GP} & \multicolumn{2}{c|}{MGP} \\ \hline
     & Error & Time & Error & Time \\ \hline
    First case & 0.1439 & $1.2$ & 0.1564 & $1.6\times10^{-1}$ \\ 
    \hline
  \end{tabular}
\end{table}

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/combcontour.pdf}
		\caption{Contours of $F_1$ on the test $x-y$ plane.}  \label{combcontour}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.6}{figures/combscatter.pdf}
		\caption{Original test output versus learned result for $F_1$. Red regions are $\pm\sqrt{\lambda}$ from the diagonal, i.e. the optimised estimate of the input noise.}  \label{combscatter}
\end{figure}

\begin{figure}[ht]
	\centering
	\pic{0.8}{figures/combslice.pdf}
		\caption{$F_1$ as a function of $x$ for constant values of $y$ and $z$. Dashed black lines are from DNS. Red regions are one standard deviation for the output.}  \label{combslice}
\end{figure}

